Financial Adviser Misconduct and Labor Market Penalties: Uncovering Racial Disparities in the Absence of Gender Gaps

Using a comprehensive matched employer-employee dataset for U.S. financial advisers from 2008 to 2018, we revisit established evidence on labor market penalties following financial misconduct. Prior studies report that female advisers are 20% more likely to exit their firms following misconduct and that similar disparities exist for non-white advisers. However, by disaggregating misconduct into distinct disclosure events - differentiating those that nearly always trigger job terminations from those that do not - we show that the apparent gender gap vanishes, while significant racial disparities persist. Specifically, non-white advisers face approximately 24% higher job separation rates than their white counterparts. Robustness checks confirm these findings across alternative specifications, suggesting that race-based differential treatment in the labor market is a distinct phenomenon warranting further investigation.

==> tables/table_1_.tex <==
\multicolumn{7}{c}{\specialcell{\bf A. Adviser Characteristics}}\\
\midrule
&\multicolumn{3}{c}{\specialcell{Male}}&\multicolumn{3}{c}{\specialcell{Female}}\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
          &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
          &\multicolumn{1}{c}{\specialcell{All}}&\multicolumn{1}{c}{\specialcell{Majority}}&\multicolumn{1}{c}{\specialcell{Minority}}&\multicolumn{1}{c}{\specialcell{All}}&\multicolumn{1}{c}{\specialcell{Majority}}&\multicolumn{1}{c}{\specialcell{Minority}}\\
\midrule
{\specialcell{\bf Employment History and Status:}}&         &         &         &         &         &         \\
\ \specialcell{Experience (years)}&     13.4&     13.9&      9.3&     10.8&     11.2&      8.1\\
\ \specialcell{Tenure (years)}&      6.3&      6.5&      4.6&      5.7&      5.9&      4.5\\
\hline {\specialcell{\bf Licenses/Industry Exams} (\%)}&         &         &         &         &         &         \\
\ \specialcell{Series 63 (General Securities Agent)}&     74.3&     74.8&     70.4&     68.7&     68.9&     67.9\\
\ \specialcell{Series 7 (General Securities Representative)}&     69.0&     69.8&     61.4&     62.4&     63.6&     55.1\\
\ \specialcell{Series 6 (Insurance and Annuities)}&     35.5&     35.2&     38.6&     42.4&     42.0&     45.2\\
\ \specialcell{Series 65/66 (Investment Adviser)}&     42.1&     43.4&     31.0&     34.8&     36.0&     27.1\\
\ \specialcell{Series 24 (Principal/Supervisory Management)}&     15.4&     16.0&     10.3&     10.6&     11.2&      7.1\\
\hline \ \specialcell{Total Number of Licenses}&      2.9&      2.9&      2.5&      2.5&      2.6&      2.3\\
\midrule
\multicolumn{7}{c}{\specialcell{\bf B. Disclosure Event Incidence}}\\
\midrule
{\specialcell{\bf Misconduct Related Disclosure Events} (\%):}&         &         &         &         &         &         \\
\ \specialcell{Customer Disputes - Settled}&     0.37&     0.37&     0.34&     0.13&     0.13&     0.12\\
\ \specialcell{Employment Separation After Allegations}&     0.23&     0.21&     0.37&     0.15&     0.14&     0.24\\
\ \specialcell{Regulatory - Final}&     0.12&     0.12&     0.12&     0.04&     0.04&     0.04\\
\ \specialcell{Criminal Disposition - Final}&     0.03&     0.03&     0.04&     0.01&     0.01&     0.01\\
\ \specialcell{Customer Disputes - Award/Judgment}&     0.02&     0.02&     0.02&     0.01&     0.01&     0.00\\
\ \specialcell{Civil - Final}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Any Misconduct Related Disclosure}&     0.71&     0.70&     0.82&     0.32&     0.31&     0.39\\
\hline {\specialcell{\bf Other Disclosure Events} (\%):}&         &         &         &         &         &         \\
\ \specialcell{Financial - Final}&     0.42&     0.40&     0.51&     0.49&     0.47&     0.58\\
\ \specialcell{Judgment/Lien}&     0.33&     0.33&     0.39&     0.20&     0.18&     0.28\\
\ \specialcell{Customer Disputes - Denied}&     0.33&     0.34&     0.27&     0.14&     0.14&     0.14\\
\ \specialcell{Customer Disputes - Closed-No Action}&     0.07&     0.07&     0.07&     0.02&     0.02&     0.03\\
\ \specialcell{Financial - Pending}&     0.04&     0.04&     0.05&     0.06&     0.05&     0.07\\
\ \specialcell{Customer Disputes - Pending}&     0.06&     0.06&     0.11&     0.02&     0.02&     0.03\\
\ \specialcell{Customer Disputes - Withdrawn}&     0.02&     0.02&     0.02&     0.01&     0.01&     0.01\\
\ \specialcell{Criminal - Pending}&     0.01&     0.01&     0.01&     0.00&     0.00&     0.01\\
\ \specialcell{Investigation}&     0.01&     0.01&     0.01&     0.00&     0.00&     0.00\\
\ \specialcell{Regulatory - Pending}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Civil - Pending}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Customer Disputes - Final}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Customer Disputes - Dismissed}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Civil Bond}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Regulatory - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Criminal - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Civil - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\hline  \specialcell{\bf Total} (\%):&     1.89&     1.86&     2.13&     1.21&     1.17&     1.46\\
\midrule
Observations&5,753,021&5,150,027&  542,597&2,153,206&1,843,251&  267,990\\


==> tables/table_1_1.tex <==
          &\multicolumn{2}{c}{\specialcell{\scriptsize Male}}&\multicolumn{2}{c}{\specialcell{\scriptsize Female}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}
          &\multicolumn{1}{c}{\specialcell{\scriptsize Majority (White)}}&\multicolumn{1}{c}{\specialcell{\scriptsize Minority (Non-White)}}&\multicolumn{1}{c}{\specialcell{\scriptsize Majority (White)}}&\multicolumn{1}{c}{\specialcell{\scriptsize Minority (Non-White)}}\\
\midrule
{\specialcell{\scriptsize \bf Employment History and Status:}}&         &         &         &         \\
\ \specialcell{\scriptsize Experience (years)}&     13.7&     11.4&     11.0&      9.4\\
\ \specialcell{\scriptsize Tenure (years)}&      6.4&      5.3&      5.8&      5.0\\
\ \specialcell{\scriptsize Currently Registered (in 2018)}&     72.4&     69.5&     69.9&     68.1\\
\hline {\specialcell{\scriptsize \bf Job Transitions (\%):}}&         &         &         &         \\
\hline \ \specialcell{\scriptsize (1) Remain at a Firm}&     83.5&     81.6&     83.7&     82.4\\
\quad \quad \ \specialcell{\scriptsize \#Advisers}&  8,511.8&  8,914.7&  9,923.5& 10,232.6\\
\quad \quad \ \specialcell{\scriptsize Total Assets (in millions of US dollars)}& 33,423.4& 53,489.9& 37,916.4& 60,008.3\\
\quad \quad \ \specialcell{\scriptsize Revenue (in millions of US dollars)}&  1,594.4&  2,229.6&  1,887.6&  2,565.4\\
\quad \quad \ \specialcell{\scriptsize AUM (in millions of US dollars)}& 80,417.9& 82,262.5& 91,622.4& 90,372.7\\
\quad \quad \ \specialcell{\scriptsize Number of Client Accounts (in thousands)}&    408.5&    395.4&    458.8&    431.9\\
\ \specialcell{\scriptsize (2) Leave a Firm}&     16.5&     18.4&     16.3&     17.6\\
\hline \quad {\specialcell{\scriptsize \bf Conditional on Leaving a Firm:}}&         &         &         &         \\
\hline \quad \ \specialcell{\scriptsize New Employment (\%)}&     50.6&     47.3&     44.1&     41.7\\
\hline  \quad \ {\specialcell{\scriptsize \bf Conditional on Finding a New Job:}}&         &         &         &         \\
\quad \quad \specialcell{\scriptsize Experience}&     12.6&     10.6&     10.3&      9.0\\
\quad \quad \specialcell{\scriptsize Tenure}&      4.8&      4.2&      4.6&      4.2\\
\quad \quad {\specialcell{\scriptsize \bf Original Firm Size:}}&         &         &         &         \\
\quad \quad \ \specialcell{\scriptsize \#Advisers}&  7,380.1&  7,702.6&  8,973.4&  9,138.5\\
\quad \quad \ \specialcell{\scriptsize Total Assets (in millions of US dollars)}& 49,606.0& 61,021.0& 59,640.7& 73,110.6\\
\quad \quad \ \specialcell{\scriptsize Revenue (in millions of US dollars)}&  2,406.5&  2,738.2&  3,212.0&  3,453.5\\
\quad \quad \ \specialcell{\scriptsize AUM (in millions of US dollars)}& 58,688.2& 60,287.1& 64,023.9& 65,515.1\\
\quad \quad \ \specialcell{\scriptsize Number of Client Accounts (in thousands)}&    306.3&    305.4&    332.1&    330.0\\
\quad \quad {\specialcell{\scriptsize \bf New Firm Size:}}&         &         &         &         \\
\quad \quad \ \specialcell{\scriptsize \#Advisers}&  7,627.0&  8,058.6& 10,066.3& 10,266.6\\
\quad \quad \ \specialcell{\scriptsize Total Assets (in millions of US dollars)}& 33,111.6& 47,621.9& 42,439.3& 59,775.7\\
\quad \quad \ \specialcell{\scriptsize Revenue (in millions of US dollars)}&  1,612.0&  2,070.9&  2,105.4&  2,569.5\\
\quad \quad \ \specialcell{\scriptsize AUM (in millions of US dollars)}& 74,051.2& 76,730.9& 89,306.7& 86,876.9\\
\quad \quad \ \specialcell{\scriptsize Number of Client Accounts (in thousands)}&    407.1&    404.4&    488.7&    459.0\\
\quad \quad {\specialcell{\scriptsize \bf Migration Across (\%):}}&         &         &         &         \\
\quad \quad \quad \specialcell{\scriptsize States}&     24.4&     21.8&     21.2&     18.5\\
\quad \quad \quad \specialcell{\scriptsize Commuting Zones}&     31.5&     28.0&     27.8&     24.6\\
\quad \quad \quad \specialcell{\scriptsize Counties}&     42.6&     38.7&     38.8&     34.7\\
\hline {\specialcell{\scriptsize \bf Licenses/Qualifications (\%):}}&         &         &         &         \\
\ \specialcell{\scriptsize Series 63 (General Securities Agent)}&     74.7&     71.7&     68.7&     68.8\\
\ \specialcell{\scriptsize Series 7 (General Securities Representative)}&     69.2&     67.3&     62.6&     61.2\\
\ \specialcell{\scriptsize Series 6 (Insurance and Annuities)}&     35.9&     32.8&     42.8&     39.9\\
\ \specialcell{\scriptsize Series 65/66 (Investment Adviser)}&     43.1&     35.5&     35.4&     30.4\\
\ \specialcell{\scriptsize Series 24 (Principal/Supervisory Management)}&     15.8&     13.2&     10.8&      8.8\\
\hline \ \specialcell{\scriptsize Total Number of Licenses}&      2.9&      2.7&      2.6&      2.4\\
\midrule
Observations&5,010,508&  742,513&1,877,475&  275,731\\


==> tables/table_1_1_1.tex <==
          &\multicolumn{3}{c}{\specialcell{Male}}&\multicolumn{3}{c}{\specialcell{Female}}\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
          &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
          &\multicolumn{1}{c}{\specialcell{All}}&\multicolumn{1}{c}{\specialcell{Majority}}&\multicolumn{1}{c}{\specialcell{Minority}}&\multicolumn{1}{c}{\specialcell{All}}&\multicolumn{1}{c}{\specialcell{Majority}}&\multicolumn{1}{c}{\specialcell{Minority}}\\
\midrule
{\specialcell{\bf Employment History and Status:}}&         &         &         &         &         &         \\
\ \specialcell{Experience (years)}&     13.4&     13.9&      9.3&     10.8&     11.2&      8.1\\
\ \specialcell{Tenure (years)}&      6.3&      6.5&      4.6&      5.7&      5.9&      4.5\\
\ \specialcell{Currently Registered (in 2018)}&     72.0&     72.5&     67.7&     69.6&     70.0&     67.7\\
\hline {\specialcell{\bf Licenses/Industry Exams}}&         &         &         &         &         &         \\
\ \specialcell{Series 63 (General Securities Agent)}&     74.3&     74.8&     70.4&     68.7&     68.9&     67.9\\
\ \specialcell{Series 7 (General Securities Representative)}&     69.0&     69.8&     61.4&     62.4&     63.6&     55.1\\
\ \specialcell{Series 6 (Insurance and Annuities)}&     35.5&     35.2&     38.6&     42.4&     42.0&     45.2\\
\ \specialcell{Series 65/66 (Investment Adviser)}&     42.1&     43.4&     31.0&     34.8&     36.0&     27.1\\
\ \specialcell{Series 24 (Principal/Supervisory Management)}&     15.4&     16.0&     10.3&     10.6&     11.2&      7.1\\
\hline \ \specialcell{Total Number of Licenses}&      2.9&      2.9&      2.5&      2.5&      2.6&      2.3\\
\midrule
Observations&5,753,021&5,150,027&  542,597&2,153,206&1,843,251&  267,990\\


==> tables/table_1_1_2.tex <==
          &\multicolumn{3}{c}{\specialcell{Male}}&\multicolumn{3}{c}{\specialcell{Female}}\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
          &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
          &\multicolumn{1}{c}{\specialcell{All}}&\multicolumn{1}{c}{\specialcell{Majority}}&\multicolumn{1}{c}{\specialcell{Minority}}&\multicolumn{1}{c}{\specialcell{All}}&\multicolumn{1}{c}{\specialcell{Majority}}&\multicolumn{1}{c}{\specialcell{Minority}}\\
\midrule
{\specialcell{\bf Employment History and Status:}}&         &         &         &         &         &         \\
\ \specialcell{Experience (years)}&     13.4&     13.9&      9.3&     10.8&     11.2&      8.1\\
\ \specialcell{Tenure (years)}&      6.3&      6.5&      4.6&      5.7&      5.9&      4.5\\
\ \specialcell{Currently Registered (in 2018)}&     72.0&     72.5&     67.7&     69.6&     70.0&     67.7\\
{\specialcell{\bf Job Transitions} (\%):}&         &         &         &         &         &         \\
\ \specialcell{(1) Remain at a Firm}&     83.2&     83.6&     80.3&     83.6&     83.9&     81.6\\
\ \specialcell{(2) Leave a Firm}&     16.8&     16.4&     19.7&     16.4&     16.1&     18.4\\
\quad {\specialcell{\bf Conditional on Leaving a Firm:}}&         &         &         &         &         &         \\
\quad \ \specialcell{(3) New Employment}&     50.1&     50.8&     44.8&     43.8&     44.3&     40.5\\
\quad \quad {\specialcell{\bf Migration Across}}&         &         &         &         &         &         \\
\quad \quad \quad \quad \specialcell{States}&     24.0&     24.5&     20.4&     20.8&     21.2&     18.1\\
\quad \quad \quad \quad \specialcell{Commuting Zones}&     31.1&     31.6&     27.0&     27.4&     27.9&     24.1\\
\quad \quad \quad \quad \specialcell{Counties}&     42.1&     42.6&     38.5&     38.3&     38.9&     34.5\\
\hline {\specialcell{\bf Licenses/Industry Exams}}&         &         &         &         &         &         \\
\ \specialcell{Series 63 (General Securities Agent)}&     74.3&     74.8&     70.4&     68.7&     68.9&     67.9\\
\ \specialcell{Series 7 (General Securities Representative)}&     69.0&     69.8&     61.4&     62.4&     63.6&     55.1\\
\ \specialcell{Series 6 (Insurance and Annuities)}&     35.5&     35.2&     38.6&     42.4&     42.0&     45.2\\
\ \specialcell{Series 65/66 (Investment Adviser)}&     42.1&     43.4&     31.0&     34.8&     36.0&     27.1\\
\ \specialcell{Series 24 (Principal/Supervisory Management)}&     15.4&     16.0&     10.3&     10.6&     11.2&      7.1\\
\hline \ \specialcell{Total Number of Licenses}&      2.9&      2.9&      2.5&      2.5&      2.6&      2.3\\
\midrule
Observations&5,753,021&5,150,027&  542,597&2,153,206&1,843,251&  267,990\\


==> tables/table_1_2.tex <==
          &\multicolumn{2}{c}{\specialcell{\scriptsize Exit Before 2008}}&\multicolumn{2}{c}{\specialcell{\scriptsize Exit After 2008}}&\multicolumn{2}{c}{\specialcell{\scriptsize Non-Exit Before 2008}}&\multicolumn{2}{c}{\specialcell{\scriptsize Non-Exit After 2008}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
          &\multicolumn{1}{c}{\specialcell{\scriptsize Male}}&\multicolumn{1}{c}{\specialcell{\scriptsize Female}}&\multicolumn{1}{c}{\specialcell{\scriptsize Male}}&\multicolumn{1}{c}{\specialcell{\scriptsize Female}}&\multicolumn{1}{c}{\specialcell{\scriptsize Male}}&\multicolumn{1}{c}{\specialcell{\scriptsize Female}}&\multicolumn{1}{c}{\specialcell{\scriptsize Male}}&\multicolumn{1}{c}{\specialcell{\scriptsize Female}}\\
\midrule
{\specialcell{\scriptsize \bf Misconduct Related Disclosure Events (\%):}}&         &         &         &         &         &         &         &         \\
\ \specialcell{\scriptsize Customer Disputes - Settled}&     0.55&     0.19&     0.07&     0.03&     0.44&     0.16&     0.05&     0.02\\
\ \specialcell{\scriptsize Employment Separation After Allegations}&     0.57&     0.34&     0.68&     0.50&     0.09&     0.05&     0.08&     0.04\\
\ \specialcell{\scriptsize Regulatory - Final}&     0.30&     0.09&     0.12&     0.06&     0.08&     0.03&     0.03&     0.01\\
\ \specialcell{\scriptsize Criminal Disposition - Final}&     0.05&     0.02&     0.05&     0.02&     0.02&     0.01&     0.02&     0.01\\
\ \specialcell{\scriptsize Customer Disputes - Award/Judgment}&     0.04&     0.01&     0.00&     0.00&     0.02&     0.01&     0.00&     0.00\\
\ \specialcell{\scriptsize Civil - Final}&     0.01&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\hline \ \specialcell{\scriptsize Any Misconduct Related Disclosure}&     1.35&     0.60&     0.85&     0.57&     0.62&     0.25&     0.18&     0.09\\
\hline {\specialcell{\scriptsize \bf Other Disclosure Events (\%):}}&         &         &         &         &         &         &         &         \\
\ \specialcell{\scriptsize Financial - Final}&     0.49&     0.48&     0.45&     0.52&     0.40&     0.50&     0.37&     0.46\\
\ {\specialcell{\scriptsize \bf Conditional on Financial - Final:}}&         &         &         &         &         &         &         &         \\
\quad \specialcell{\scriptsize Bankruptcy}&    54.32&    56.21&    45.11&    48.24&    42.01&    46.28&    30.24&    37.00\\
\quad {\specialcell{\scriptsize \bf Conditional on Bankruptcy:}}&         &         &         &         &         &         &         &         \\
\quad \quad \specialcell{\scriptsize Chapter 7}&    78.73&    75.94&    84.11&    83.78&    73.72&    72.85&    78.71&    78.51\\
\quad \quad \specialcell{\scriptsize Chapter 13}&    16.86&    18.91&    13.54&    14.17&    22.87&    24.56&    19.75&    20.13\\
\quad \ {\specialcell{\scriptsize \bf Disposition:}}&         &         &         &         &         &         &         &         \\
\quad \quad \specialcell{\scriptsize Discharged}&    83.40&    84.65&    87.64&    84.77&    84.16&    85.95&    83.53&    82.30\\
\ \specialcell{\scriptsize Customer Disputes - Denied}&     0.36&     0.16&     0.04&     0.02&     0.44&     0.20&     0.08&     0.03\\
\ \specialcell{\scriptsize Judgment/Lien}&     0.52&     0.25&     0.28&     0.22&     0.33&     0.19&     0.15&     0.15\\
\ \specialcell{\scriptsize Customer Disputes - Closed-No Action}&     0.12&     0.03&     0.02&     0.01&     0.08&     0.03&     0.02&     0.01\\
\ \specialcell{\scriptsize Financial - Pending}&     0.08&     0.09&     0.10&     0.12&     0.03&     0.03&     0.03&     0.05\\
\ \specialcell{\scriptsize Customer Disputes - Pending}&     0.11&     0.03&     0.02&     0.00&     0.06&     0.02&     0.02&     0.01\\
\ \specialcell{\scriptsize Customer Disputes - Withdrawn}&     0.02&     0.01&     0.00&     0.00&     0.02&     0.01&     0.00&     0.00\\
\ \specialcell{\scriptsize Criminal - Pending}&     0.03&     0.01&     0.04&     0.02&     0.00&     0.00&     0.01&     0.00\\
\ \specialcell{\scriptsize Investigation}&     0.02&     0.01&     0.01&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{\scriptsize Regulatory - Pending}&     0.01&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{\scriptsize Civil - Pending}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{\scriptsize Customer Disputes - Final}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{\scriptsize Customer Disputes - Dismissed}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{\scriptsize Civil Bond}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{\scriptsize Regulatory - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{\scriptsize Criminal - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{\scriptsize Civil - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\hline  \specialcell{\scriptsize Total of All Disclosure Events}&     2.84&     1.59&     1.74&     1.43&     1.90&     1.19&     0.82&     0.77\\
\midrule
Observations&1,169,609&  461,188&  438,841&  192,671&3,139,796&1,056,330&1,004,775&  443,017\\


==> tables/table_1_2_1.tex <==
          &\multicolumn{3}{c}{\specialcell{Male}}&\multicolumn{3}{c}{\specialcell{Female}}\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
          &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
          &\multicolumn{1}{c}{\specialcell{All}}&\multicolumn{1}{c}{\specialcell{Majority}}&\multicolumn{1}{c}{\specialcell{Minority}}&\multicolumn{1}{c}{\specialcell{All}}&\multicolumn{1}{c}{\specialcell{Majority}}&\multicolumn{1}{c}{\specialcell{Minority}}\\
\midrule
{\specialcell{\bf Misconduct Related Disclosure Events} (\%):}&         &         &         &         &         &         \\
\ \specialcell{Customer Disputes - Settled}&     0.37&     0.37&     0.34&     0.13&     0.13&     0.12\\
\ \specialcell{Employment Separation After Allegations}&     0.23&     0.21&     0.37&     0.15&     0.14&     0.24\\
\quad {\specialcell{\it Conditional on Employment Separation:}}&         &         &         &         &         &         \\
\quad \quad \specialcell{Discharged}&    77.27&    76.69&    79.99&    83.47&    83.28&    85.02\\
\quad \quad \specialcell{Voluntary Resign}&    11.07&    11.89&     6.79&     6.50&     6.94&     4.42\\
\quad \quad \specialcell{Permitted to Resign}&    11.68&    11.44&    13.23&    10.01&     9.78&    10.41\\
\ \specialcell{Regulatory - Final}&     0.12&     0.12&     0.12&     0.04&     0.04&     0.04\\
\ \specialcell{Criminal Disposition - Final}&     0.03&     0.03&     0.04&     0.01&     0.01&     0.01\\
\quad {\specialcell{\it Conditional on Criminal - Final:}}&         &         &         &         &         &         \\
\quad \quad \specialcell{Felony}&    86.99&    87.45&    82.96&    75.39&    75.76&    73.58\\
\ \specialcell{Customer Disputes - Award/Judgment}&     0.02&     0.02&     0.02&     0.01&     0.01&     0.00\\
\ \specialcell{Civil - Final}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Any Misconduct Related Disclosure}&     0.71&     0.70&     0.82&     0.32&     0.31&     0.39\\
\hline {\specialcell{\bf Other Disclosure Events} (\%):}&         &         &         &         &         &         \\
\ \specialcell{Financial - Final}&     0.42&     0.40&     0.51&     0.49&     0.47&     0.58\\
\quad {\specialcell{\it Conditional on Financial - Final:}}&         &         &         &         &         &         \\
\quad \ \specialcell{Bankruptcy}&    43.39&    43.56&    42.46&    46.77&    47.06&    45.43\\
\quad \ \specialcell{Compromise}&    56.65&    56.49&    57.54&    53.25&    52.96&    54.57\\
\quad \ {\specialcell{\it Conditional on Bankruptcy:}}&         &         &         &         &         &         \\
\quad \quad \specialcell{Chapter 7}&    76.65&    76.77&    75.95&    75.57&    75.74&    74.61\\
\quad \quad \quad {\specialcell{\it Disposition:}}&         &         &         &         &         &         \\
\quad \quad  \quad \ \specialcell{Discharged}&    96.34&    96.43&    95.68&    96.59&    96.78&    95.61\\
\quad \quad \specialcell{Chapter 13}&    19.93&    19.73&    21.01&    21.42&    21.17&    22.79\\
\quad \quad \quad {\specialcell{\it Disposition:}}&         &         &         &         &         &         \\
\quad \quad  \quad \ \specialcell{Discharged}&    87.93&    88.30&    85.64&    87.91&    88.31&    85.84\\
\ \specialcell{Customer Disputes - Denied}&     0.33&     0.34&     0.27&     0.14&     0.14&     0.14\\
\ \specialcell{Judgment/Lien}&     0.33&     0.33&     0.39&     0.20&     0.18&     0.28\\
\quad \specialcell{\it Conditional on Judgment/Lien}&         &         &         &         &         &         \\
\quad \quad \specialcell{Civil}&    64.31&    65.40&    56.19&    48.21&    50.88&    37.26\\
\quad \quad \specialcell{Tax}&    35.69&    34.60&    43.81&    51.79&    49.12&    62.74\\
\ \specialcell{Customer Disputes - Closed-No Action}&     0.07&     0.07&     0.07&     0.02&     0.02&     0.03\\
\ \specialcell{Financial - Pending}&     0.04&     0.04&     0.05&     0.06&     0.05&     0.07\\
\ \specialcell{Customer Disputes - Pending}&     0.06&     0.06&     0.11&     0.02&     0.02&     0.03\\
\ \specialcell{Customer Disputes - Withdrawn}&     0.02&     0.02&     0.02&     0.01&     0.01&     0.01\\
\ \specialcell{Criminal - Pending}&     0.01&     0.01&     0.01&     0.00&     0.00&     0.01\\
\ \specialcell{Investigation}&     0.01&     0.01&     0.01&     0.00&     0.00&     0.00\\
\ \specialcell{Regulatory - Pending}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Civil - Pending}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Customer Disputes - Final}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Customer Disputes - Dismissed}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Civil Bond}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Regulatory - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Criminal - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Civil - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\hline  \specialcell{\bf Total} (\%):&     1.89&     1.86&     2.13&     1.21&     1.17&     1.46\\
\midrule
Observations&5,753,021&5,150,027&  542,597&2,153,206&1,843,251&  267,990\\


==> tables/table_1_2_2.tex <==
          &\multicolumn{3}{c}{\specialcell{Male}}&\multicolumn{3}{c}{\specialcell{Female}}\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
          &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
          &\multicolumn{1}{c}{\specialcell{All}}&\multicolumn{1}{c}{\specialcell{Majority}}&\multicolumn{1}{c}{\specialcell{Minority}}&\multicolumn{1}{c}{\specialcell{All}}&\multicolumn{1}{c}{\specialcell{Majority}}&\multicolumn{1}{c}{\specialcell{Minority}}\\
\midrule
{\specialcell{\bf Misconduct Related Disclosure Events} (\%):}&         &         &         &         &         &         \\
\ \specialcell{Customer Disputes - Settled}&     0.37&     0.37&     0.34&     0.13&     0.13&     0.12\\
\ \specialcell{Employment Separation After Allegations}&     0.23&     0.21&     0.37&     0.15&     0.14&     0.24\\
\ \specialcell{Regulatory - Final}&     0.12&     0.12&     0.12&     0.04&     0.04&     0.04\\
\ \specialcell{Criminal Disposition - Final}&     0.03&     0.03&     0.04&     0.01&     0.01&     0.01\\
\ \specialcell{Customer Disputes - Award/Judgment}&     0.02&     0.02&     0.02&     0.01&     0.01&     0.00\\
\ \specialcell{Civil - Final}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Any Misconduct Related Disclosure}&     0.71&     0.70&     0.82&     0.32&     0.31&     0.39\\
\hline {\specialcell{\bf Other Disclosure Events} (\%):}&         &         &         &         &         &         \\
\ \specialcell{Financial - Final}&     0.42&     0.40&     0.51&     0.49&     0.47&     0.58\\
\ \specialcell{Judgment/Lien}&     0.33&     0.33&     0.39&     0.20&     0.18&     0.28\\
\ \specialcell{Customer Disputes - Denied}&     0.33&     0.34&     0.27&     0.14&     0.14&     0.14\\
\ \specialcell{Customer Disputes - Closed-No Action}&     0.07&     0.07&     0.07&     0.02&     0.02&     0.03\\
\ \specialcell{Financial - Pending}&     0.04&     0.04&     0.05&     0.06&     0.05&     0.07\\
\ \specialcell{Customer Disputes - Pending}&     0.06&     0.06&     0.11&     0.02&     0.02&     0.03\\
\ \specialcell{Customer Disputes - Withdrawn}&     0.02&     0.02&     0.02&     0.01&     0.01&     0.01\\
\ \specialcell{Criminal - Pending}&     0.01&     0.01&     0.01&     0.00&     0.00&     0.01\\
\ \specialcell{Investigation}&     0.01&     0.01&     0.01&     0.00&     0.00&     0.00\\
\ \specialcell{Regulatory - Pending}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Civil - Pending}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Customer Disputes - Final}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Customer Disputes - Dismissed}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Civil Bond}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Regulatory - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Criminal - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Civil - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\hline  \specialcell{\bf Total} (\%):&     1.89&     1.86&     2.13&     1.21&     1.17&     1.46\\
\midrule
Observations&5,753,021&5,150,027&  542,597&2,153,206&1,843,251&  267,990\\


==> tables/table_2_1_1.tex <==
          &\multicolumn{1}{c}{\specialcell{\scriptsize No Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Cus.Set.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Emp.Sep.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Reg.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Others}}\\
\midrule
{\specialcell{\scriptsize \bf Job Transitions (\%):}}&         &         &         &         &         &         \\
\ \specialcell{\scriptsize Remain at a Firm}&     83.8&     53.5&     74.4&      4.7&     52.1&     65.4\\
\ \specialcell{\scriptsize Leave a Firm}&     16.2&     46.5&     25.6&     95.3&     47.9&     34.6\\
\hline \quad {\specialcell{\scriptsize \it Conditional on Leaving a Firm:}}&         &         &         &         &         &         \\
\quad \ \specialcell{\scriptsize Join a New Firm}&     51.0&     43.0&     63.1&     34.6&     23.0&     44.1\\
\quad \ \specialcell{\scriptsize Not Finding a Job}&     49.0&     57.0&     36.9&     65.4&     77.0&     55.9\\
\midrule
Observations&4,545,523&   35,009&   18,792&   10,570&    5,798&    2,364\\


==> tables/table_2_1_2.tex <==
          &\multicolumn{1}{c}{\specialcell{\scriptsize No Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Cus.Set.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Emp.Sep.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Reg.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Others}}\\
\midrule
{\specialcell{\scriptsize \bf Job Transitions (\%):}}&         &         &         &         &         &         \\
\ \specialcell{\scriptsize Remain at a Firm}&     80.6&     40.8&     70.4&      4.1&     40.2&     64.4\\
\ \specialcell{\scriptsize Leave a Firm}&     19.4&     59.2&     29.6&     95.9&     59.8&     35.6\\
\hline \quad {\specialcell{\scriptsize \it Conditional on Leaving a Firm:}}&         &         &         &         &         &         \\
\quad \ \specialcell{\scriptsize Join a New Firm}&     45.2&     32.5&     58.6&     25.1&     16.1&     43.5\\
\quad \ \specialcell{\scriptsize Not Finding a Job}&     54.8&     67.5&     41.4&     74.9&     83.9&     56.5\\
\midrule
Observations&  470,696&    4,306&    1,822&    1,925&      622&      303\\


==> tables/table_2_2_1.tex <==
          &\multicolumn{1}{c}{\specialcell{\scriptsize No Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Cus.Set.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Emp.Sep.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Reg.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Others}}\\
\midrule
{\specialcell{\scriptsize \bf Job Transitions (\%):}}&         &         &         &         &         &         \\
\ \specialcell{\scriptsize Remain at a Firm}&     84.0&     44.4&     75.7&      4.6&     52.8&     71.4\\
\ \specialcell{\scriptsize Leave a Firm}&     16.0&     55.6&     24.3&     95.4&     47.2&     28.6\\
\hline \quad {\specialcell{\scriptsize \it Conditional on Leaving a Firm:}}&         &         &         &         &         &         \\
\quad \ \specialcell{\scriptsize Join a New Firm}&     44.5&     31.5&     57.7&     25.1&     15.8&     50.6\\
\quad \ \specialcell{\scriptsize Not Finding a Job}&     55.5&     68.5&     42.3&     74.9&     84.2&     49.4\\
\midrule
Observations&1,635,782&    5,527&    2,302&    2,437&      779&      304\\


==> tables/table_2_2_2.tex <==
          &\multicolumn{1}{c}{\specialcell{\scriptsize No Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Cus.Set.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Emp.Sep.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Reg.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Others}}\\
\midrule
{\specialcell{\scriptsize \bf Job Transitions (\%):}}&         &         &         &         &         &         \\
\ \specialcell{\scriptsize Remain at a Firm}&     81.9&     32.2&     72.0&      5.4&     35.0&     78.3\\
\ \specialcell{\scriptsize Leave a Firm}&     18.1&     67.8&     28.0&     94.6&     65.0&     21.7\\
\hline \quad {\specialcell{\scriptsize \it Conditional on Leaving a Firm:}}&         &         &         &         &         &         \\
\quad \ \specialcell{\scriptsize Join a New Firm}&     40.8&     22.3&     57.8&     17.8&      7.7&     40.0\\
\quad \ \specialcell{\scriptsize Not Finding a Job}&     59.2&     77.7&     42.2&     82.2&     92.3&     60.0\\
\midrule
Observations&  234,797&    1,031&      321&      616&      100&       46\\


==> tables/table_2_js_0_1.tex <==
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}     \\
\midrule
\ \specialcell{\scriptsize Female}&    -0.22         &    -0.85\sym{***}&    -0.31\sym{**} &    -0.26\sym{**} \\
                &   (0.24)         &   (0.27)         &   (0.14)         &   (0.13)               \\
\addlinespace
\ \specialcell{\scriptsize Misconduct}&    31.47\sym{***}&    32.16\sym{***}&    27.69\sym{***}&    29.24\sym{***}\\
                &   (1.76)         &   (1.65)         &   (1.90)         &   (2.20)             \\
\addlinespace
\ \specialcell{\scriptsize Female $\times$ Misconduct}&     9.72\sym{***}&     9.68\sym{***}&    11.04\sym{***}&    10.94\sym{***}\\
                &   (1.68)         &   (1.55)         &   (1.58)         &   (1.57)          \\
\midrule
\specialcell{\scriptsize Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                 \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$                \\
\specialcell{\scriptsize Observations}&7,022,703         &7,022,703         &6,571,326         &5,736,702             \\
\specialcell{\scriptsize \(R^2\)}&    0.005         &    0.017         &    0.260         &    0.316            \\
\specialcell{\scriptsize Mean of Dependent Variable}&    16.66         &    16.66         &    16.81         &    16.58             \\


==> tables/table_2_js_0_1_0.tex <==
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
\ \specialcell{\scriptsize Female}&    -0.22         &    -1.07\sym{***}&    -0.81\sym{***}&    -0.31\sym{**} &    -0.36\sym{***}&    -0.44\sym{***}\\
                &   (0.24)         &   (0.25)         &   (0.13)         &   (0.13)         &   (0.14)         &   (0.15)         \\
\addlinespace
\ \specialcell{\scriptsize Disclosure}&    31.47\sym{***}&    31.55\sym{***}&    27.01\sym{***}&    29.26\sym{***}&    34.41\sym{***}&    39.04\sym{***}\\
                &   (1.76)         &   (1.61)         &   (1.83)         &   (2.20)         &   (3.08)         &   (3.84)         \\
\addlinespace
\ \specialcell{\scriptsize Female $\times$ Disclosure}&     9.72\sym{***}&     9.47\sym{***}&    10.82\sym{***}&    10.94\sym{***}&    10.07\sym{***}&     9.10\sym{***}\\
                &   (1.68)         &   (1.54)         &   (1.56)         &   (1.58)         &   (1.42)         &   (1.44)         \\
\addlinespace
\ \specialcell{\scriptsize Experience}&                  &    -0.39\sym{***}&    -0.40\sym{***}&    -0.38\sym{***}&                  &                  \\
                &                  &   (0.07)         &   (0.05)         &   (0.06)         &                  &                  \\
\addlinespace
\ \specialcell{\scriptsize Experience$^{2}$}&                  &     0.01\sym{***}&     0.01\sym{***}&     0.01\sym{***}&                  &                  \\
                &                  &   (0.00)         &   (0.00)         &   (0.00)         &                  &                  \\
\addlinespace
\ \specialcell{\scriptsize Tenure}&                  &    -0.43\sym{***}&    -0.29\sym{***}&    -0.23\sym{***}&    -0.14\sym{***}&                  \\
                &                  &   (0.05)         &   (0.03)         &   (0.04)         &   (0.04)         &                  \\
\addlinespace
\ \specialcell{\scriptsize Series 65/66}&                  &     3.88\sym{***}&     3.49\sym{***}&                  &                  &                  \\
                &                  &   (0.41)         &   (0.31)         &                  &                  &                  \\
\addlinespace
\ \specialcell{\scriptsize registered with SEC}&                  &   -11.23\sym{***}&   -10.79\sym{***}&                  &                  &                  \\
                &                  &   (0.82)         &   (0.72)         &                  &                  &                  \\
\addlinespace
\ \specialcell{\scriptsize Series 63}&                  &    -0.34         &    -0.40\sym{**} &                  &                  &                  \\
                &                  &   (0.38)         &   (0.20)         &                  &                  &                  \\
\addlinespace
\ \specialcell{\scriptsize Series 7}&                  &     0.85         &     0.57\sym{**} &                  &                  &                  \\
                &                  &   (0.71)         &   (0.28)         &                  &                  &                  \\
\addlinespace
\ \specialcell{\scriptsize Series 6}&                  &    -0.13         &     0.13         &                  &                  &                  \\
                &                  &   (0.61)         &   (0.27)         &                  &                  &                  \\
\addlinespace
\ \specialcell{\scriptsize Series 24}&                  &    -0.95         &    -1.59\sym{***}&                  &                  &                  \\
                &                  &   (0.64)         &   (0.25)         &                  &                  &                  \\
\addlinespace
\ \specialcell{\scriptsize Number of Other Licenses}&                  &    -0.18         &    -0.28\sym{***}&    -0.28\sym{***}&    -0.38\sym{**} &    -0.67\sym{***}\\
                &                  &   (0.24)         &   (0.08)         &   (0.09)         &   (0.15)         &   (0.23)         \\
\addlinespace
\ \specialcell{\scriptsize Certified Financial Planner}&                  &     2.23\sym{***}&     1.86\sym{***}&    -2.10\sym{***}&    -1.40         &    -1.70         \\
                &                  &   (0.84)         &   (0.61)         &   (0.60)         &   (1.01)         &   (1.18)         \\
\addlinespace
\ \specialcell{\scriptsize Certified Financial Analyst}&                  &     6.34\sym{***}&     6.27\sym{***}&     0.47         &     1.34         &     1.10         \\
                &                  &   (0.92)         &   (0.64)         &   (0.67)         &   (0.95)         &   (1.16)         \\
\addlinespace
\ \specialcell{\scriptsize Certified Financial Consultant}&                  &     0.60         &     0.93         &    -3.88\sym{***}&    -4.22\sym{***}&    -4.74\sym{***}\\
                &                  &   (0.78)         &   (0.70)         &   (0.42)         &   (0.71)         &   (0.52)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                  &                  &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$         &                  &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &                  &                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience $\times$ Tenure FE}&                  &                  &                  &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&7,022,703         &7,022,703         &6,571,326         &5,736,702         &3,463,871         &2,555,364         \\
\specialcell{\scriptsize \(R^2\)}&    0.005         &    0.031         &    0.270         &    0.316         &    0.406         &    0.417         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    16.66         &    16.66         &    16.81         &    16.58         &    16.67         &    17.13         \\


==> tables/table_2_js_0_1_1.tex <==
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
\ \specialcell{\scriptsize Female}&    -0.22         &    -1.07\sym{***}&    -0.81\sym{***}&    -0.31\sym{**} &    -0.36\sym{***}&    -0.44\sym{***}\\
                &   (0.24)         &   (0.25)         &   (0.13)         &   (0.13)         &   (0.14)         &   (0.15)         \\
\addlinespace
\ \specialcell{\scriptsize Disclosure}&    31.47\sym{***}&    31.55\sym{***}&    27.01\sym{***}&    29.26\sym{***}&    34.41\sym{***}&    39.04\sym{***}\\
                &   (1.76)         &   (1.61)         &   (1.83)         &   (2.20)         &   (3.08)         &   (3.84)         \\
\addlinespace
\ \specialcell{\scriptsize Female $\times$ Disclosure}&     9.72\sym{***}&     9.47\sym{***}&    10.82\sym{***}&    10.94\sym{***}&    10.07\sym{***}&     9.10\sym{***}\\
                &   (1.68)         &   (1.54)         &   (1.56)         &   (1.58)         &   (1.42)         &   (1.44)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                  &                  &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$         &                  &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience FE}&                  &                  &                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License $\times$ Experience $\times$ Tenure FE}&                  &                  &                  &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&7,022,703         &7,022,703         &6,571,326         &5,736,702         &3,463,871         &2,555,364         \\
\specialcell{\scriptsize \(R^2\)}&    0.005         &    0.031         &    0.270         &    0.316         &    0.406         &    0.417         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    16.66         &    16.66         &    16.81         &    16.58         &    16.67         &    17.13         \\


==> tables/table_2_js_1_1.tex <==
                &\multicolumn{2}{c}{\specialcell{Misconduct}}&\multicolumn{2}{c}{\specialcell{A}}  &\multicolumn{2}{c}{\specialcell{B}}  \\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
\ \specialcell{Female}&    -0.85\sym{***}&    -0.26\sym{**} &    -0.86\sym{***}&    -0.24\sym{*}  &    -0.89\sym{***}&    -0.30\sym{**} \\
                &   (0.27)         &   (0.13)         &   (0.27)         &   (0.13)         &   (0.27)         &   (0.13)         \\
\addlinespace
\ \specialcell{Disclosure}&    32.16\sym{***}&    29.24\sym{***}&    78.36\sym{***}&    74.92\sym{***}&    15.42\sym{***}&    10.02\sym{***}\\
                &   (1.65)         &   (2.20)         &   (0.73)         &   (1.40)         &   (0.85)         &   (0.73)         \\
\addlinespace
\ \specialcell{Female $\times$ Disclosure}&     9.68\sym{***}&    10.94\sym{***}&     0.08         &     0.87         &    -0.36         &    -0.03         \\
                &   (1.55)         &   (1.57)         &   (0.56)         &   (0.80)         &   (0.89)         &   (0.90)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{Observations}&7,022,703         &5,736,702         &7,022,703         &5,736,702         &7,022,703         &5,736,702         \\
\specialcell{\(R^2\)}&    0.017         &    0.316         &    0.022         &    0.320         &    0.013         &    0.312         \\
\specialcell{Mean of Dependent Variable}&    16.66         &    16.58         &    16.66         &    16.58         &    16.66         &    16.58         \\


==> tables/table_2_js_1_3.tex <==
                &\multicolumn{5}{c}{\specialcell{\scriptsize Job Separation (\%)}}                             \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                &\multicolumn{1}{c}{\specialcell{\scriptsize Set $ A $}}&\multicolumn{1}{c}{\specialcell{\scriptsize (I)}}&\multicolumn{1}{c}{\specialcell{\scriptsize (II)}}&\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct (excl. (II))}}\\
\midrule
\ \specialcell{\scriptsize Female}&    -0.27\sym{**} &    -0.31\sym{**} &    -0.24\sym{*}  &    -0.26\sym{**} &    -0.30\sym{**} \\
                &   (0.13)         &   (0.13)         &   (0.13)         &   (0.13)         &   (0.13)         \\
\addlinespace
\ \specialcell{\scriptsize Disclosure}&    32.82\sym{***}&     6.44\sym{***}&    74.92\sym{***}&    29.24\sym{***}&    10.02\sym{***}\\
                &   (2.52)         &   (0.62)         &   (1.40)         &   (2.20)         &   (0.73)         \\
\addlinespace
\ \specialcell{\scriptsize Female $\times$ Disclosure}&    12.24\sym{***}&    -1.15         &     0.87         &    10.94\sym{***}&    -0.03         \\
                &   (1.52)         &   (0.83)         &   (0.80)         &   (1.57)         &   (0.90)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&5,736,702         &5,736,702         &5,736,702         &5,736,702         &5,736,702         \\
\specialcell{\scriptsize \(R^2\)}&    0.316         &    0.312         &    0.320         &    0.316         &    0.312         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    16.58         &    16.58         &    16.58         &    16.58         &    16.58         \\


==> tables/table_2_js_1_4.tex <==
                &\multicolumn{4}{c}{\specialcell{\scriptsize Job Separation (\%)}}                             \\\cmidrule(lr){2-5}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                &\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct (excl. (II))}}&\multicolumn{1}{c}{\specialcell{\scriptsize (I)}}&\multicolumn{1}{c}{\specialcell{\scriptsize (II)}}\\
\midrule
\ \specialcell{\scriptsize Female}&    -0.26\sym{**} &    -0.30\sym{**} &    -0.31\sym{**} &    -0.24\sym{*}   \\
              &   (0.13)         &   (0.13)         &   (0.13)         &   (0.13)                 \\
\addlinespace
\ \specialcell{\scriptsize Disclosure}&    29.24\sym{***}&    10.02\sym{***}&     6.44\sym{***}&    74.92\sym{***}\\
                  &   (2.20)         &   (0.73)          &   (0.62)         &   (1.40)               \\
\addlinespace
\ \specialcell{\scriptsize Female $\times$ Disclosure}&    10.94\sym{***}&    -0.03&    -1.15         &     0.87                  \\
               &   (1.57)         &   (0.90)      &   (0.83)         &   (0.80)                  \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                \\
\specialcell{\scriptsize Observations}&5,736,702         &5,736,702         &5,736,702         &5,736,702           \\
\specialcell{\scriptsize \(R^2\)}&    0.316         &    0.312        &    0.312         &    0.320                  \\
\specialcell{\scriptsize Mean of Dependent Variable}&    16.58         &    16.58         &    16.58         &    16.58           \\


==> tables/table_2_js_2_0_1.tex <==
                &\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct (excl. Emp.Sep.)}}&\multicolumn{1}{c}{\specialcell{\scriptsize Cus.Set.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Emp.Sep.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Reg.}}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
\specialcell{\scriptsize Disclosure}&    27.86\sym{***}&     4.57\sym{***}&     6.20\sym{***}&    75.03\sym{***}&    25.08\sym{***}\\
                &   (1.91)         &   (0.46)         &   (0.62)         &   (1.43)         &   (2.11)         \\
\addlinespace
\specialcell{\scriptsize Hispanic}&     0.19         &     0.29         &     0.29         &     0.27         &     0.29         \\
                &   (0.21)         &   (0.20)         &   (0.20)         &   (0.20)         &   (0.20)         \\
\addlinespace
\specialcell{\scriptsize Asian}&     0.73\sym{***}&     0.84\sym{***}&     0.83\sym{***}&     0.79\sym{***}&     0.84\sym{***}\\
                &   (0.20)         &   (0.18)         &   (0.18)         &   (0.19)         &   (0.18)         \\
\addlinespace
\specialcell{\scriptsize Black}&     0.45\sym{**} &     0.50\sym{***}&     0.50\sym{***}&     0.47\sym{**} &     0.49\sym{**} \\
                &   (0.19)         &   (0.19)         &   (0.19)         &   (0.19)         &   (0.19)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Hispanic}&    10.04\sym{***}&     2.43\sym{**} &     2.97\sym{**} &    -3.08         &     9.06\sym{***}\\
                &   (3.17)         &   (1.22)         &   (1.33)         &   (2.09)         &   (3.00)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Asian}&    14.76\sym{***}&     1.00         &     5.41\sym{**} &     1.56         &    10.92\sym{**} \\
                &   (2.59)         &   (1.84)         &   (2.20)         &   (1.20)         &   (4.58)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Black}&     5.76\sym{**} &     0.72         &     0.57         &    -1.15         &     7.62         \\
                &   (2.76)         &   (2.93)         &   (3.28)         &   (3.42)         &   (7.28)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&4,002,487         &4,002,487         &4,002,487         &4,002,487         &4,002,487         \\
\specialcell{\scriptsize \(R^2\)}&    0.328         &    0.325         &    0.325         &    0.333         &    0.325         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    16.67         &    16.67         &    16.67         &    16.67         &    16.67         \\


==> tables/table_2_js_2_0_2.tex <==
                &\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct (excl. Emp.Sep.)}}&\multicolumn{1}{c}{\specialcell{\scriptsize Cus.Set.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Emp.Sep.}}&\multicolumn{1}{c}{\specialcell{\scriptsize Reg.}}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
\specialcell{\scriptsize Disclosure}&    41.19\sym{***}&     4.62\sym{***}&     5.59\sym{***}&    77.39\sym{***}&    29.19\sym{***}\\
                &   (3.85)         &   (1.24)         &   (1.50)         &   (1.63)         &   (6.65)         \\
\addlinespace
\specialcell{\scriptsize Hispanic}&    -0.51\sym{***}&    -0.48\sym{***}&    -0.47\sym{***}&    -0.48\sym{***}&    -0.48\sym{***}\\
                &   (0.18)         &   (0.17)         &   (0.17)         &   (0.17)         &   (0.17)         \\
\addlinespace
\specialcell{\scriptsize Asian}&     0.75\sym{***}&     0.83\sym{***}&     0.84\sym{***}&     0.77\sym{***}&     0.83\sym{***}\\
                &   (0.25)         &   (0.25)         &   (0.25)         &   (0.25)         &   (0.25)         \\
\addlinespace
\specialcell{\scriptsize Black}&     0.08         &     0.10         &     0.10         &     0.10         &     0.11         \\
                &   (0.23)         &   (0.23)         &   (0.23)         &   (0.23)         &   (0.23)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Hispanic}&     8.25\sym{**} &     4.64         &     1.66         &    -6.82\sym{**} &    20.24\sym{***}\\
                &   (3.33)         &   (3.24)         &   (4.64)         &   (2.96)         &   (6.65)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Asian}&     9.52\sym{***}&     1.34         &     0.27         &    -5.17\sym{**} &    26.92\sym{*}  \\
                &   (3.23)         &   (4.24)         &   (3.93)         &   (2.38)         &  (14.48)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Black}&     1.99         &     0.78         &     4.33         &    -2.84         &    -9.84         \\
                &   (6.80)         &   (8.33)         &  (13.88)         &   (7.80)         &  (14.87)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&1,417,189         &1,417,189         &1,417,189         &1,417,189         &1,417,189         \\
\specialcell{\scriptsize \(R^2\)}&    0.337         &    0.333         &    0.333         &    0.339         &    0.334         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    16.07         &    16.07         &    16.07         &    16.07         &    16.07         \\


==> tables/table_2_js_2_1.tex <==
                &\multicolumn{1}{c}{\specialcell{Misconduct}}&\multicolumn{1}{c}{\specialcell{$ A $}}&\multicolumn{1}{c}{\specialcell{$ B $}}&\multicolumn{1}{c}{\specialcell{(I)}}&\multicolumn{1}{c}{\specialcell{(III)}}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}\cmidrule(lr){6-6}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
\specialcell{Minority}&     0.57\sym{***}&     0.63\sym{***}&     0.66\sym{***}&     0.67\sym{***}&     0.67\sym{***}\\
                &   (0.19)         &   (0.18)         &   (0.18)         &   (0.18)         &   (0.18)         \\
\addlinespace
\specialcell{Disclosure}&    29.14\sym{***}&    75.36\sym{***}&     9.36\sym{***}&     5.89\sym{***}&    25.21\sym{***}\\
                &   (2.09)         &   (1.39)         &   (0.69)         &   (0.64)         &   (2.28)         \\
\addlinespace
\specialcell{Minority $ \times $ Disclosure}&    13.76\sym{***}&    -1.52         &     6.41\sym{***}&     4.41\sym{***}&    12.44\sym{***}\\
                &   (2.48)         &   (1.29)         &   (1.40)         &   (1.30)         &   (2.84)         \\
\addlinespace
\specialcell{Female}&    -0.23\sym{*}  &    -0.25\sym{*}  &    -0.31\sym{**} &    -0.33\sym{**} &    -0.33\sym{**} \\
                &   (0.13)         &   (0.13)         &   (0.13)         &   (0.13)         &   (0.13)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Observations}&5,736,702         &5,736,702         &5,736,702         &5,736,702         &5,736,702         \\
\specialcell{\(R^2\)}&    0.316         &    0.320         &    0.312         &    0.312         &    0.312         \\
\specialcell{Mean of Dependent Variable}&    16.58         &    16.58         &    16.58         &    16.58         &    16.58         \\


==> tables/table_3_in_1.tex <==
                &\multicolumn{3}{c}{\specialcell{Incidence of $ A$(\%)}} &\multicolumn{3}{c}{\specialcell{Incidence of $ B$(\%)}} \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
\specialcell{Female}&    -0.11\sym{***}&    -0.09\sym{***}&    -0.08\sym{***}&    -0.23\sym{***}&    -0.20\sym{***}&    -0.14\sym{***}\\
                &   (0.02)         &   (0.02)         &   (0.02)         &   (0.03)         &   (0.03)         &   (0.02)         \\
\addlinespace
\specialcell{$ B$(\%)}&                  &     0.07\sym{***}&     0.07\sym{***}&                  &                  &                  \\
                &                  &   (0.01)         &   (0.01)         &                  &                  &                  \\
\addlinespace
\specialcell{Female $ \times $ $ B$(\%)}&                  &     0.00         &     0.00         &                  &                  &                  \\
                &                  &   (0.01)         &   (0.01)         &                  &                  &                  \\
\addlinespace
\specialcell{$ B^{Prior} $}&                  &                  &     0.25\sym{***}&                  &                  &     1.27\sym{***}\\
                &                  &                  &   (0.02)         &                  &                  &   (0.07)         \\
\addlinespace
\specialcell{$ A^{Prior} $}&                  &                  &     0.43\sym{***}&                  &                  &     1.98\sym{***}\\
                &                  &                  &   (0.06)         &                  &                  &   (0.12)         \\
\addlinespace
\specialcell{Female $ \times $  $ B^{Prior} $}&                  &                  &    -0.05\sym{*}  &                  &                  &    -0.45\sym{***}\\
                &                  &                  &   (0.03)         &                  &                  &   (0.08)         \\
\addlinespace
\specialcell{Female $ \times $  $ A^{Prior} $}&                  &                  &    -0.03         &                  &                  &    -0.20         \\
                &                  &                  &   (0.13)         &                  &                  &   (0.27)         \\
\addlinespace
\specialcell{$ A$(\%)}&                  &                  &                  &                  &     0.14\sym{***}&     0.14\sym{***}\\
                &                  &                  &                  &                  &   (0.01)         &   (0.01)         \\
\addlinespace
\specialcell{Female $ \times $  $ A$(\%)}&                  &                  &                  &                  &    -0.06\sym{***}&    -0.06\sym{***}\\
                &                  &                  &                  &                  &   (0.01)         &   (0.01)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Observations}&6,273,000         &6,273,000         &6,273,000         &6,273,000         &6,273,000         &6,273,000         \\
\specialcell{\(R^2\)}&    0.139         &    0.146         &    0.147         &    0.189         &    0.196         &    0.199         \\
\specialcell{Mean of Dependent Variable}&     0.21         &     0.21         &     0.21         &     0.40         &     0.40         &     0.40         \\


==> tables/table_3_in_2.tex <==
                &\multicolumn{3}{c}{\specialcell{Incidence of $ A$(\%)}} &\multicolumn{3}{c}{\specialcell{Incidence of $ B$(\%)}} \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
\specialcell{Minority}&     0.07\sym{***}&     0.05\sym{***}&     0.05\sym{***}&     0.02\sym{**} &     0.02\sym{*}  &     0.00         \\
                &   (0.01)         &   (0.01)         &   (0.01)         &   (0.01)         &   (0.01)         &   (0.01)         \\
\addlinespace
\specialcell{Female}&    -0.11\sym{***}&    -0.09\sym{***}&    -0.08\sym{***}&    -0.23\sym{***}&    -0.21\sym{***}&    -0.17\sym{***}\\
                &   (0.02)         &   (0.02)         &   (0.02)         &   (0.03)         &   (0.03)         &   (0.02)         \\
\addlinespace
\specialcell{$ B$(\%)}&                  &     0.07\sym{***}&     0.07\sym{***}&                  &                  &                  \\
                &                  &   (0.01)         &   (0.01)         &                  &                  &                  \\
\addlinespace
\specialcell{Minority $ \times $ $ B$(\%)}&                  &     0.05\sym{***}&     0.05\sym{***}&                  &                  &                  \\
                &                  &   (0.01)         &   (0.01)         &                  &                  &                  \\
\addlinespace
\specialcell{$ B^{Prior} $}&                  &                  &     0.23\sym{***}&                  &                  &     1.19\sym{***}\\
                &                  &                  &   (0.02)         &                  &                  &   (0.06)         \\
\addlinespace
\specialcell{$ A^{Prior} $}&                  &                  &     0.41\sym{***}&                  &                  &     1.96\sym{***}\\
                &                  &                  &   (0.05)         &                  &                  &   (0.13)         \\
\addlinespace
\specialcell{Minority $ \times $  $ B^{Prior} $}&                  &                  &     0.09\sym{*}  &                  &                  &     0.22         \\
                &                  &                  &   (0.05)         &                  &                  &   (0.21)         \\
\addlinespace
\specialcell{Minority $ \times $  $ A^{Prior} $}&                  &                  &     0.19         &                  &                  &     0.11         \\
                &                  &                  &   (0.18)         &                  &                  &   (0.37)         \\
\addlinespace
\specialcell{$ A$(\%)}&                  &                  &                  &                  &     0.13\sym{***}&     0.13\sym{***}\\
                &                  &                  &                  &                  &   (0.01)         &   (0.01)         \\
\addlinespace
\specialcell{Minority $ \times $  $ A$(\%)}&                  &                  &                  &                  &    -0.02\sym{**} &    -0.02\sym{**} \\
                &                  &                  &                  &                  &   (0.01)         &   (0.01)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Observations}&6,273,000         &6,273,000         &6,273,000         &6,273,000         &6,273,000         &6,273,000         \\
\specialcell{\(R^2\)}&    0.139         &    0.147         &    0.147         &    0.189         &    0.196         &    0.198         \\
\specialcell{Mean of Dependent Variable}&     0.21         &     0.21         &     0.21         &     0.40         &     0.40         &     0.40         \\


==> tables/table_4_1.tex <==
                &\multicolumn{5}{c}{\specialcell{New Employment(\%)}}                                          \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                &\multicolumn{1}{c}{\specialcell{Misconduct}}&\multicolumn{1}{c}{\specialcell{Misconduct(excl.Emp.Sep.)}}&\multicolumn{1}{c}{\specialcell{Cus.Set.}}&\multicolumn{1}{c}{\specialcell{Emp.Sep.}}&\multicolumn{1}{c}{\specialcell{Reg.}}\\
\midrule
\specialcell{Disclosure}&   -12.09\sym{***}&    -2.92         &     0.58         &   -13.56\sym{***}&   -20.29\sym{***}\\
                &   (1.66)         &   (3.14)         &   (3.26)         &   (1.92)         &   (5.66)         \\
\addlinespace
\specialcell{Hispanic}&     1.14\sym{**} &     1.07\sym{**} &     1.06\sym{**} &     1.09\sym{**} &     1.07\sym{**} \\
                &   (0.53)         &   (0.52)         &   (0.52)         &   (0.53)         &   (0.52)         \\
\addlinespace
\specialcell{Asian}&    -2.00\sym{**} &    -2.01\sym{**} &    -2.03\sym{**} &    -2.03\sym{**} &    -2.02\sym{**} \\
                &   (0.83)         &   (0.82)         &   (0.82)         &   (0.83)         &   (0.82)         \\
\addlinespace
\specialcell{Black}&    -0.19         &    -0.24         &    -0.24         &    -0.18         &    -0.24         \\
                &   (0.75)         &   (0.73)         &   (0.73)         &   (0.75)         &   (0.73)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Hispanic}&    -2.31         &    -3.37         &    -1.68         &     0.04         &   -13.82         \\
                &   (5.67)         &  (10.19)         &  (10.35)         &   (6.10)         &  (16.52)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Asian}&     0.93         &   -22.08\sym{***}&    -4.75         &     4.66         &   -27.29\sym{**} \\
                &   (4.73)         &   (6.76)         &   (7.48)         &   (5.98)         &  (13.75)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Black}&    -2.41         &     4.25         &     8.32         &    -2.03         &     6.46         \\
                &   (4.25)         &  (18.53)         &  (27.08)         &   (4.42)         &  (10.77)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Observations}&  174,656         &  174,656         &  174,656         &  174,656         &  174,656         \\
\specialcell{\(R^2\)}&    0.516         &    0.516         &    0.516         &    0.516         &    0.516         \\
\specialcell{Mean of Dependent Variable}&    43.14         &    43.14         &    43.14         &    43.14         &    43.14         \\


==> tables/table_4_2_1.tex <==
                &\multicolumn{5}{c}{\specialcell{New Employment(\%)}}                                          \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                &\multicolumn{1}{c}{\specialcell{Misconduct}}&\multicolumn{1}{c}{\specialcell{Misconduct(excl.Emp.Sep.)}}&\multicolumn{1}{c}{\specialcell{Cus.Set.}}&\multicolumn{1}{c}{\specialcell{Emp.Sep.}}&\multicolumn{1}{c}{\specialcell{Reg.}}\\
\midrule
\specialcell{Disclosure}&   -10.19\sym{***}&    -1.57         &     5.23\sym{***}&   -12.82\sym{***}&   -21.98\sym{***}\\
                &   (1.23)         &   (1.16)         &   (1.24)         &   (1.44)         &   (2.14)         \\
\addlinespace
\specialcell{Hispanic}&     1.32\sym{***}&     1.17\sym{***}&     1.15\sym{***}&     1.22\sym{***}&     1.14\sym{***}\\
                &   (0.39)         &   (0.37)         &   (0.38)         &   (0.39)         &   (0.37)         \\
\addlinespace
\specialcell{Asian}&    -4.48\sym{***}&    -4.50\sym{***}&    -4.51\sym{***}&    -4.47\sym{***}&    -4.48\sym{***}\\
                &   (0.51)         &   (0.51)         &   (0.51)         &   (0.52)         &   (0.52)         \\
\addlinespace
\specialcell{Black}&    -1.29\sym{**} &    -1.44\sym{**} &    -1.44\sym{**} &    -1.32\sym{**} &    -1.42\sym{**} \\
                &   (0.58)         &   (0.58)         &   (0.58)         &   (0.57)         &   (0.58)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Hispanic}&    -5.36\sym{**} &    -4.87         &    -2.92         &    -3.12         &     1.49         \\
                &   (2.31)         &   (3.05)         &   (4.03)         &   (2.84)         &   (7.05)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Asian}&     2.56         &     5.50         &     9.56         &     2.70         &    -6.20         \\
                &   (1.88)         &   (5.74)         &   (6.29)         &   (1.81)         &  (11.27)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Black}&    -4.11\sym{*}  &     2.33         &     2.88         &    -5.60\sym{*}  &   -13.27         \\
                &   (2.33)         &   (5.08)         &   (5.60)         &   (3.10)         &   (8.57)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Observations}&  539,245         &  539,245         &  539,245         &  539,245         &  539,245         \\
\specialcell{\(R^2\)}&    0.454         &    0.453         &    0.453         &    0.454         &    0.454         \\
\specialcell{Mean of Dependent Variable}&    51.15         &    51.15         &    51.15         &    51.15         &    51.15         \\


==> tables/table_4_2_2.tex <==
                &\multicolumn{5}{c}{\specialcell{New Employment(\%)}}                                          \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                &\multicolumn{1}{c}{\specialcell{Misconduct}}&\multicolumn{1}{c}{\specialcell{Misconduct(excl.Emp.Sep.)}}&\multicolumn{1}{c}{\specialcell{Cus.Set.}}&\multicolumn{1}{c}{\specialcell{Emp.Sep.}}&\multicolumn{1}{c}{\specialcell{Reg.}}\\
\midrule
\specialcell{Disclosure}&   -12.09\sym{***}&    -2.92         &     0.58         &   -13.56\sym{***}&   -20.29\sym{***}\\
                &   (1.66)         &   (3.14)         &   (3.26)         &   (1.92)         &   (5.66)         \\
\addlinespace
\specialcell{Hispanic}&     1.14\sym{**} &     1.07\sym{**} &     1.06\sym{**} &     1.09\sym{**} &     1.07\sym{**} \\
                &   (0.53)         &   (0.52)         &   (0.52)         &   (0.53)         &   (0.52)         \\
\addlinespace
\specialcell{Asian}&    -2.00\sym{**} &    -2.01\sym{**} &    -2.03\sym{**} &    -2.03\sym{**} &    -2.02\sym{**} \\
                &   (0.83)         &   (0.82)         &   (0.82)         &   (0.83)         &   (0.82)         \\
\addlinespace
\specialcell{Black}&    -0.19         &    -0.24         &    -0.24         &    -0.18         &    -0.24         \\
                &   (0.75)         &   (0.73)         &   (0.73)         &   (0.75)         &   (0.73)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Hispanic}&    -2.31         &    -3.37         &    -1.68         &     0.04         &   -13.82         \\
                &   (5.67)         &  (10.19)         &  (10.35)         &   (6.10)         &  (16.52)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Asian}&     0.93         &   -22.08\sym{***}&    -4.75         &     4.66         &   -27.29\sym{**} \\
                &   (4.73)         &   (6.76)         &   (7.48)         &   (5.98)         &  (13.75)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Black}&    -2.41         &     4.25         &     8.32         &    -2.03         &     6.46         \\
                &   (4.25)         &  (18.53)         &  (27.08)         &   (4.42)         &  (10.77)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Observations}&  174,656         &  174,656         &  174,656         &  174,656         &  174,656         \\
\specialcell{\(R^2\)}&    0.516         &    0.516         &    0.516         &    0.516         &    0.516         \\
\specialcell{Mean of Dependent Variable}&    43.14         &    43.14         &    43.14         &    43.14         &    43.14         \\


==> tables/table_in_g_1.tex <==
                &\multicolumn{3}{c}{\specialcell{Event (II)}} &\multicolumn{3}{c}{\specialcell{Misconduct (excl. Event (II))}} \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
\specialcell{Female}&    -0.11\sym{***}&    -0.09\sym{***}&    -0.08\sym{***}&    -0.23\sym{***}&    -0.20\sym{***}&    -0.14\sym{***}\\
                &   (0.02)         &   (0.02)         &   (0.02)         &   (0.03)         &   (0.03)         &   (0.02)         \\
\addlinespace
\specialcell{Misconduct (excl. Event (II))}&                  &     0.07\sym{***}&     0.07\sym{***}&                  &                  &                  \\
                &                  &   (0.01)         &   (0.01)         &                  &                  &                  \\
\addlinespace
\specialcell{Misconduct (excl. Event (II)) $ \times $ Female}&                  &     0.00         &     0.00         &                  &                  &                  \\
                &                  &   (0.01)         &   (0.01)         &                  &                  &                  \\
\addlinespace
\specialcell{Misconduct (excl. Event (II))$^{\text{Prior}}$}&                  &                  &     0.25\sym{***}&                  &                  &     1.27\sym{***}\\
                &                  &                  &   (0.02)         &                  &                  &   (0.07)         \\
\addlinespace
\specialcell{Event (II)$^{\text{Prior}}$}&                  &                  &     0.43\sym{***}&                  &                  &     1.98\sym{***}\\
                &                  &                  &   (0.06)         &                  &                  &   (0.12)         \\
\addlinespace
\specialcell{Misconduct (excl. Event (II))$^{\text{Prior}}$ $ \times $ Female}&                  &                  &    -0.05\sym{*}  &                  &                  &    -0.45\sym{***}\\
                &                  &                  &   (0.03)         &                  &                  &   (0.08)         \\
\addlinespace
\specialcell{Event (II)$^{\text{Prior}}$ $ \times $  Female}&                  &                  &    -0.03         &                  &                  &    -0.20         \\
                &                  &                  &   (0.13)         &                  &                  &   (0.27)         \\
\addlinespace
\specialcell{Event (II)}&                  &                  &                  &                  &     0.14\sym{***}&     0.14\sym{***}\\
                &                  &                  &                  &                  &   (0.01)         &   (0.01)         \\
\addlinespace
\specialcell{Event (II) $ \times $ Female}&                  &                  &                  &                  &    -0.06\sym{***}&    -0.06\sym{***}\\
                &                  &                  &                  &                  &   (0.01)         &   (0.01)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Observations}&6,273,000         &6,273,000         &6,273,000         &6,273,000         &6,273,000         &6,273,000         \\
\specialcell{\(R^2\)}&    0.139         &    0.146         &    0.147         &    0.189         &    0.196         &    0.199         \\
\specialcell{Mean of Dependent Variable}&     0.21         &     0.21         &     0.21         &     0.40         &     0.40         &     0.40         \\


==> tables/table_in_g_2.tex <==
                &\multicolumn{3}{c}{\specialcell{Incidence of Event (II)}} &\multicolumn{3}{c}{\specialcell{Incidence of Misconduct (excl. Event (II))}} \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
\specialcell{Female}&    -0.11\sym{***}&    -0.09\sym{***}&    -0.08\sym{***}&    -0.23\sym{***}&    -0.20\sym{***}&    -0.14\sym{***}\\
                &   (0.02)         &   (0.02)         &   (0.02)         &   (0.03)         &   (0.03)         &   (0.02)         \\
\addlinespace
\specialcell{Misconduct (excl. Event (II))}&                  &     0.07\sym{***}&     0.07\sym{***}&                  &                  &                  \\
                &                  &   (0.01)         &   (0.01)         &                  &                  &                  \\
\addlinespace
\specialcell{Female $ \times $ Misconduct (excl. Event (II))}&                  &     0.00         &     0.00         &                  &                  &                  \\
                &                  &   (0.01)         &   (0.01)         &                  &                  &                  \\
\addlinespace
\specialcell{Misconduct (excl. Event (II))$^{\text{Prior}}$}&                  &                  &     0.25\sym{***}&                  &                  &     1.27\sym{***}\\
                &                  &                  &   (0.02)         &                  &                  &   (0.07)         \\
\addlinespace
\specialcell{Event (II)$^{\text{Prior}}$}&                  &                  &     0.43\sym{***}&                  &                  &     1.98\sym{***}\\
                &                  &                  &   (0.06)         &                  &                  &   (0.12)         \\
\addlinespace
\specialcell{$\text{Misconduct (excl. Event (II))}^{\text{Prior}} \times \text{Female} $}&                  &                  &    -0.05\sym{*}  &                  &                  &    -0.45\sym{***}\\
                &                  &                  &   (0.03)         &                  &                  &   (0.08)         \\
\addlinespace
\specialcell{$\text{Event (II)}^{\text{Prior}} \times \text{Female}$}&                  &                  &    -0.03         &                  &                  &    -0.20         \\
                &                  &                  &   (0.13)         &                  &                  &   (0.27)         \\
\addlinespace
\specialcell{Event (II)}&                  &                  &                  &                  &     0.14\sym{***}&     0.14\sym{***}\\
                &                  &                  &                  &                  &   (0.01)         &   (0.01)         \\
\addlinespace
\specialcell{Female $ \times $  Event (II)}&                  &                  &                  &                  &    -0.06\sym{***}&    -0.06\sym{***}\\
                &                  &                  &                  &                  &   (0.01)         &   (0.01)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Observations}&6,273,000         &6,273,000         &6,273,000         &6,273,000         &6,273,000         &6,273,000         \\
\specialcell{\(R^2\)}&    0.139         &    0.146         &    0.147         &    0.189         &    0.196         &    0.199         \\
\specialcell{Mean of Dependent Variable}&     0.21         &     0.21         &     0.21         &     0.40         &     0.40         &     0.40         \\


==> tables/table_in_r_1.tex <==
                &\multicolumn{3}{c}{\specialcell{Incidence of $ A$(\%)}} &\multicolumn{3}{c}{\specialcell{Incidence of $ B$(\%)}} \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
\specialcell{Minority}&     0.07\sym{***}&     0.05\sym{***}&     0.05\sym{***}&     0.02\sym{**} &     0.02\sym{*}  &     0.00         \\
                &   (0.01)         &   (0.01)         &   (0.01)         &   (0.01)         &   (0.01)         &   (0.01)         \\
\addlinespace
\specialcell{Female}&    -0.11\sym{***}&    -0.09\sym{***}&    -0.08\sym{***}&    -0.23\sym{***}&    -0.21\sym{***}&    -0.17\sym{***}\\
                &   (0.02)         &   (0.02)         &   (0.02)         &   (0.03)         &   (0.03)         &   (0.02)         \\
\addlinespace
\specialcell{$ B$(\%)}&                  &     0.07\sym{***}&     0.07\sym{***}&                  &                  &                  \\
                &                  &   (0.01)         &   (0.01)         &                  &                  &                  \\
\addlinespace
\specialcell{Minority $ \times $ $ B$(\%)}&                  &     0.05\sym{***}&     0.05\sym{***}&                  &                  &                  \\
                &                  &   (0.01)         &   (0.01)         &                  &                  &                  \\
\addlinespace
\specialcell{$ B^{Prior} $}&                  &                  &     0.23\sym{***}&                  &                  &     1.19\sym{***}\\
                &                  &                  &   (0.02)         &                  &                  &   (0.06)         \\
\addlinespace
\specialcell{$ A^{Prior} $}&                  &                  &     0.41\sym{***}&                  &                  &     1.96\sym{***}\\
                &                  &                  &   (0.05)         &                  &                  &   (0.13)         \\
\addlinespace
\specialcell{Minority $ \times $  $ B^{Prior} $}&                  &                  &     0.09\sym{*}  &                  &                  &     0.22         \\
                &                  &                  &   (0.05)         &                  &                  &   (0.21)         \\
\addlinespace
\specialcell{Minority $ \times $  $ A^{Prior} $}&                  &                  &     0.19         &                  &                  &     0.11         \\
                &                  &                  &   (0.18)         &                  &                  &   (0.37)         \\
\addlinespace
\specialcell{$ A$(\%)}&                  &                  &                  &                  &     0.13\sym{***}&     0.13\sym{***}\\
                &                  &                  &                  &                  &   (0.01)         &   (0.01)         \\
\addlinespace
\specialcell{Minority $ \times $  $ A$(\%)}&                  &                  &                  &                  &    -0.02\sym{**} &    -0.02\sym{**} \\
                &                  &                  &                  &                  &   (0.01)         &   (0.01)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Observations}&6,273,000         &6,273,000         &6,273,000         &6,273,000         &6,273,000         &6,273,000         \\
\specialcell{\(R^2\)}&    0.139         &    0.147         &    0.147         &    0.189         &    0.196         &    0.198         \\
\specialcell{Mean of Dependent Variable}&     0.21         &     0.21         &     0.21         &     0.40         &     0.40         &     0.40         \\


==> tables/table_in_r_2.tex <==
                &\multicolumn{3}{c}{\specialcell{Event (II)}} &\multicolumn{3}{c}{\specialcell{Misconduct (excl. Event (II))}} \\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\midrule
\specialcell{Minority}&     0.07\sym{***}&     0.05\sym{***}&     0.05\sym{***}&     0.02\sym{**} &     0.02\sym{*}  &     0.00         \\
                &   (0.01)         &   (0.01)         &   (0.01)         &   (0.01)         &   (0.01)         &   (0.01)         \\
\addlinespace
\specialcell{Misconduct (excl. Event (II))}&                  &     0.07\sym{***}&     0.07\sym{***}&                  &                  &                  \\
                &                  &   (0.01)         &   (0.01)         &                  &                  &                  \\
\addlinespace
\specialcell{Misconduct (excl. Event (II)) $ \times $ Minority}&                  &     0.05\sym{***}&     0.05\sym{***}&                  &                  &                  \\
                &                  &   (0.01)         &   (0.01)         &                  &                  &                  \\
\addlinespace
\specialcell{Misconduct (excl. Event (II))$^{\text{Prior}}$}&                  &                  &     0.23\sym{***}&                  &                  &     1.19\sym{***}\\
                &                  &                  &   (0.02)         &                  &                  &   (0.06)         \\
\addlinespace
\specialcell{Event (II)$^{\text{Prior}}$}&                  &                  &     0.41\sym{***}&                  &                  &     1.96\sym{***}\\
                &                  &                  &   (0.05)         &                  &                  &   (0.13)         \\
\addlinespace
\specialcell{$\text{Misconduct (excl. Event (II))}^{\text{Prior}} \times \text{Minority}$}&                  &                  &     0.09\sym{*}  &                  &                  &     0.22         \\
                &                  &                  &   (0.05)         &                  &                  &   (0.21)         \\
\addlinespace
\specialcell{$\text{Event (II)}^{\text{Prior}} \times \text{Minority}$}&                  &                  &     0.19         &                  &                  &     0.11         \\
                &                  &                  &   (0.18)         &                  &                  &   (0.37)         \\
\addlinespace
\specialcell{Event (II)}&                  &                  &                  &                  &     0.13\sym{***}&     0.13\sym{***}\\
                &                  &                  &                  &                  &   (0.01)         &   (0.01)         \\
\addlinespace
\specialcell{$\text{Event (II)} \times \text{Minority}$}&                  &                  &                  &                  &    -0.02\sym{**} &    -0.02\sym{**} \\
                &                  &                  &                  &                  &   (0.01)         &   (0.01)         \\
\addlinespace
\specialcell{Female}&    -0.11\sym{***}&    -0.09\sym{***}&    -0.08\sym{***}&    -0.23\sym{***}&    -0.21\sym{***}&    -0.17\sym{***}\\
                &   (0.02)         &   (0.02)         &   (0.02)         &   (0.03)         &   (0.03)         &   (0.02)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Observations}&6,273,000         &6,273,000         &6,273,000         &6,273,000         &6,273,000         &6,273,000         \\
\specialcell{\(R^2\)}&    0.139         &    0.147         &    0.147         &    0.189         &    0.196         &    0.198         \\
\specialcell{Mean of Dependent Variable}&     0.21         &     0.21         &     0.21         &     0.40         &     0.40         &     0.40         \\


==> tables/table_js_1_g_1_0.tex <==
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}     \\
\midrule
\ \specialcell{\scriptsize Female}&    -0.22         &    -0.85\sym{***}&    -0.31\sym{**} &    -0.26\sym{**} \\
                &   (0.24)         &   (0.27)         &   (0.14)         &   (0.13)               \\
\addlinespace
\ \specialcell{\scriptsize Misconduct}&    31.47\sym{***}&    32.16\sym{***}&    27.69\sym{***}&    29.24\sym{***}\\
                &   (1.76)         &   (1.65)         &   (1.90)         &   (2.20)             \\
\addlinespace
\ \specialcell{\scriptsize Female $\times$ Misconduct}&     9.72\sym{***}&     9.68\sym{***}&    11.04\sym{***}&    10.94\sym{***}\\
                &   (1.68)         &   (1.55)         &   (1.58)         &   (1.57)          \\
\midrule
\specialcell{\scriptsize Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                 \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$                \\
\specialcell{\scriptsize Observations}&7,022,703         &7,022,703         &6,571,326         &5,736,702             \\
\specialcell{\scriptsize \(R^2\)}&    0.005         &    0.017         &    0.260         &    0.316            \\
\specialcell{\scriptsize Mean of Dependent Variable}&    16.66         &    16.66         &    16.81         &    16.58             \\


==> tables/table_js_1_g_1_1.tex <==
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}     \\
\midrule
\ \specialcell{Female}&    -0.22         &    -0.85\sym{***}&    -0.31\sym{**} &    -0.26\sym{**} \\
                &   (0.24)         &   (0.27)         &   (0.14)         &   (0.13)               \\
\addlinespace
\ \specialcell{Misconduct}&    31.47\sym{***}&    32.16\sym{***}&    27.69\sym{***}&    29.24\sym{***}\\
                &   (1.76)         &   (1.65)         &   (1.90)         &   (2.20)             \\
\addlinespace
% \ \specialcell{Female $\times$ Misconduct}&     9.72\sym{***}&     9.68\sym{***}&    11.04\sym{***}&    10.94\sym{***}\\
\ \specialcell{Misconduct $\times$ Female}&     9.72\sym{***}&     9.68\sym{***}&    11.04\sym{***}&    10.94\sym{***}\\
                &   (1.68)         &   (1.55)         &   (1.58)         &   (1.57)          \\
\midrule
\specialcell{Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                \\
\specialcell{Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                 \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$                \\
\specialcell{Observations}&7,022,703         &7,022,703         &6,571,326         &5,736,702             \\
\specialcell{\(R^2\)}&    0.005         &    0.017         &    0.260         &    0.316            \\
\specialcell{Mean of Dependent Variable}&    16.66         &    16.66         &    16.81         &    16.58             \\


==> tables/table_js_1_r_1.tex <==
                &\multicolumn{4}{c}{\specialcell{Job Separation (\%)}}                      \\\cmidrule(lr){2-5}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
\specialcell{Minority}&     2.20\sym{***}&     1.85\sym{***}&     1.60\sym{***}&     1.54\sym{***}\\
                &   (0.53)         &   (0.51)         &   (0.21)         &   (0.21)         \\
\addlinespace
\specialcell{Disclosure}&    49.64\sym{***}&    48.80\sym{***}&    48.39\sym{***}&    51.45\sym{***}\\
                &   (3.64)         &   (3.47)         &   (4.11)         &   (3.95)         \\
\addlinespace
\specialcell{Minority $ \times $ Disclosure}&    11.94\sym{***}&    11.55\sym{***}&    14.15\sym{***}&    10.46\sym{***}\\
                &   (2.48)         &   (2.50)         &   (2.42)         &   (3.09)         \\
\addlinespace
\specialcell{Female}&    -1.26\sym{***}&    -1.49\sym{***}&    -0.25         &    -0.18         \\
                &   (0.26)         &   (0.26)         &   (0.24)         &   (0.26)         \\
\midrule
\specialcell{Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{Observations}&  510,644         &  510,644         &  441,789         &  386,400         \\
\specialcell{\(R^2\)}&    0.006         &    0.011         &    0.207         &    0.248         \\
\specialcell{Mean of Dependent Variable}&    20.60         &    20.60         &    20.64         &    20.03         \\


==> tables/table_js_1_r_1_2.tex <==
                &\multicolumn{2}{c}{\specialcell{Misconduct}}&\multicolumn{2}{c}{\specialcell{$ A $}}&\multicolumn{2}{c}{\specialcell{$ B $}}&\multicolumn{2}{c}{\specialcell{(I)}}&\multicolumn{2}{c}{\specialcell{(III)}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         &\multicolumn{1}{c}{(9)}         &\multicolumn{1}{c}{(10)}         \\
\midrule
\specialcell{Minority}&     1.36\sym{***}&     0.57\sym{***}&     1.41\sym{***}&     0.63\sym{***}&     1.49\sym{***}&     0.66\sym{***}&     1.51\sym{***}&     0.67\sym{***}&     1.50\sym{***}&     0.67\sym{***}\\
                &   (0.44)         &   (0.19)         &   (0.44)         &   (0.18)         &   (0.44)         &   (0.18)         &   (0.44)         &   (0.18)         &   (0.44)         &   (0.18)         \\
\addlinespace
\specialcell{Disclosure}&    32.33\sym{***}&    29.14\sym{***}&    78.71\sym{***}&    75.36\sym{***}&    14.97\sym{***}&     9.36\sym{***}&    10.60\sym{***}&     5.89\sym{***}&    31.95\sym{***}&    25.21\sym{***}\\
                &   (1.55)         &   (2.09)         &   (0.72)         &   (1.39)         &   (0.83)         &   (0.69)         &   (1.04)         &   (0.64)         &   (1.84)         &   (2.28)         \\
\addlinespace
\specialcell{Minority $ \times $ Disclosure}&    10.36\sym{***}&    13.76\sym{***}&    -2.59\sym{***}&    -1.52         &     3.97\sym{***}&     6.41\sym{***}&     2.14         &     4.41\sym{***}&     9.84\sym{***}&    12.44\sym{***}\\
                &   (2.64)         &   (2.48)         &   (0.76)         &   (1.29)         &   (1.50)         &   (1.40)         &   (1.38)         &   (1.30)         &   (2.49)         &   (2.84)         \\
\addlinespace
\specialcell{Female}&    -0.84\sym{***}&    -0.23\sym{*}  &    -0.88\sym{***}&    -0.25\sym{*}  &    -0.91\sym{***}&    -0.31\sym{**} &    -0.94\sym{***}&    -0.33\sym{**} &    -0.94\sym{***}&    -0.33\sym{**} \\
                &   (0.26)         &   (0.13)         &   (0.26)         &   (0.13)         &   (0.26)         &   (0.13)         &   (0.26)         &   (0.13)         &   (0.26)         &   (0.13)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{Observations}&7,022,703         &5,736,702         &7,022,703         &5,736,702         &7,022,703         &5,736,702         &7,022,703         &5,736,702         &7,022,703         &5,736,702         \\
\specialcell{\(R^2\)}&    0.018         &    0.316         &    0.022         &    0.320         &    0.013         &    0.312         &    0.012         &    0.312         &    0.013         &    0.312         \\
\specialcell{Mean of Dependent Variable}&    16.66         &    16.58         &    16.66         &    16.58         &    16.66         &    16.58         &    16.66         &    16.58         &    16.66         &    16.58         \\


==> tables/table_js_1_r_1_3.tex <==
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}             \\
\midrule
\specialcell{Minority}&     1.36\sym{***}&     0.57\sym{***} \\
                &   (0.44)         &   (0.19)             \\
\addlinespace
\specialcell{Misconduct}&    32.33\sym{***}&    29.14\sym{***}\\
                &   (1.55)         &   (2.09)        \\
\addlinespace
\specialcell{Misconduct $ \times $ Minority}&    10.36\sym{***}&    13.76\sym{***}\\
                &   (2.64)         &   (2.48)           \\
\addlinespace
\specialcell{Female}&    -0.84\sym{***}&    -0.23\sym{*}   \\
                &   (0.26)         &   (0.13)             \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$            \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&                  &$\pmb{\checkmark}$                     \\
\specialcell{Observations}&7,022,703         &5,736,702          \\
\specialcell{\(R^2\)}&    0.018         &    0.316         \\
\specialcell{Mean of Dependent Variable}&    16.66         &    16.58       \\


==> tables/table_js_1_r_f_1.tex <==
                &\multicolumn{4}{c}{\specialcell{\scriptsize Job Separation (\%)}}          \\\cmidrule(lr){2-5}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
\specialcell{\scriptsize Disclosure}&    39.57\sym{***}&    39.95\sym{***}&    37.82\sym{***}&    40.52\sym{***}\\
                &   (2.72)         &   (2.60)         &   (3.10)         &   (3.76)         \\
\addlinespace
\specialcell{\scriptsize Hispanic}&     1.40\sym{**} &     0.26         &    -0.17         &    -0.36\sym{*}  \\
                &   (0.70)         &   (0.60)         &   (0.19)         &   (0.20)         \\
\addlinespace
\specialcell{\scriptsize Asian}&     3.34\sym{***}&     2.23\sym{***}&     0.66\sym{**} &     0.73\sym{**} \\
                &   (0.59)         &   (0.59)         &   (0.30)         &   (0.30)         \\
\addlinespace
\specialcell{\scriptsize Black}&     1.62\sym{***}&     0.82\sym{*}  &     0.86\sym{***}&     0.71\sym{***}\\
                &   (0.52)         &   (0.44)         &   (0.22)         &   (0.22)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Hispanic}&    11.62\sym{***}&    11.59\sym{***}&    10.72\sym{***}&    12.64\sym{***}\\
                &   (3.84)         &   (3.62)         &   (3.75)         &   (3.71)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Asian}&     8.32\sym{***}&     8.39\sym{***}&    10.22\sym{***}&     9.83\sym{***}\\
                &   (2.91)         &   (2.90)         &   (2.78)         &   (3.37)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Black}&     9.61\sym{**} &     9.45\sym{**} &    10.02\sym{**} &    15.69\sym{***}\\
                &   (4.88)         &   (4.66)         &   (4.63)         &   (3.82)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&1,914,244         &1,914,244         &1,715,081         &1,417,189         \\
\specialcell{\scriptsize \(R^2\)}&    0.005         &    0.013         &    0.279         &    0.337         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    16.43         &    16.43         &    16.44         &    16.07         \\


==> tables/table_js_1_r_m_1.tex <==
                &\multicolumn{4}{c}{\specialcell{\scriptsize Job Separation (\%)}}          \\\cmidrule(lr){2-5}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\midrule
\specialcell{\scriptsize Disclosure}&    30.40\sym{***}&    31.15\sym{***}&    26.39\sym{***}&    27.55\sym{***}\\
                &   (1.47)         &   (1.39)         &   (1.65)         &   (1.89)         \\
\addlinespace
\specialcell{\scriptsize Hispanic}&     2.84\sym{***}&     1.12\sym{*}  &     0.55\sym{**} &     0.40         \\
                &   (0.74)         &   (0.62)         &   (0.25)         &   (0.26)         \\
\addlinespace
\specialcell{\scriptsize Asian}&     4.23\sym{***}&     2.11\sym{***}&     0.74\sym{***}&     0.82\sym{***}\\
                &   (0.57)         &   (0.49)         &   (0.23)         &   (0.23)         \\
\addlinespace
\specialcell{\scriptsize Black}&     2.18\sym{***}&     1.44\sym{***}&     1.31\sym{***}&     1.13\sym{***}\\
                &   (0.58)         &   (0.43)         &   (0.22)         &   (0.25)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Hispanic}&     7.57\sym{*}  &     7.87\sym{**} &    11.13\sym{***}&    11.97\sym{***}\\
                &   (4.31)         &   (3.88)         &   (3.25)         &   (3.48)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Asian}&    13.36\sym{***}&    13.98\sym{***}&    16.29\sym{***}&    18.24\sym{***}\\
                &   (2.59)         &   (2.44)         &   (2.74)         &   (2.75)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Black}&    10.36\sym{***}&    10.17\sym{***}&    11.93\sym{***}&    12.46\sym{***}\\
                &   (2.10)         &   (2.03)         &   (2.19)         &   (2.37)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&                  &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County FE}&                  &                  &$\pmb{\checkmark}$         &                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&                  &                  &                  &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&5,108,459         &5,108,459         &4,715,333         &4,002,487         \\
\specialcell{\scriptsize \(R^2\)}&    0.006         &    0.020         &    0.270         &    0.328         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    16.75         &    16.75         &    16.90         &    16.67         \\


==> tables/table_js_1_r_r_1.tex <==
                &\multicolumn{2}{c}{\specialcell{Misconduct}}&\multicolumn{2}{c}{\specialcell{$ A $}}&\multicolumn{2}{c}{\specialcell{$ B $}}&\multicolumn{2}{c}{\specialcell{(I)}}&\multicolumn{2}{c}{\specialcell{(III)}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         &\multicolumn{1}{c}{(9)}         &\multicolumn{1}{c}{(10)}         \\
\midrule
\specialcell{Asina}&     3.93\sym{***}&     0.76\sym{***}&     3.92\sym{***}&     0.81\sym{***}&     4.01\sym{***}&     0.87\sym{***}&     4.00\sym{***}&     0.88\sym{***}&     4.00\sym{***}&     0.88\sym{***}\\
                &   (0.56)         &   (0.24)         &   (0.56)         &   (0.23)         &   (0.56)         &   (0.23)         &   (0.56)         &   (0.23)         &   (0.56)         &   (0.23)         \\
\addlinespace
\specialcell{Black}&     1.98\sym{***}&     1.15\sym{***}&     1.99\sym{***}&     1.20\sym{***}&     2.05\sym{***}&     1.23\sym{***}&     2.07\sym{***}&     1.25\sym{***}&     2.06\sym{***}&     1.24\sym{***}\\
                &   (0.54)         &   (0.20)         &   (0.54)         &   (0.20)         &   (0.55)         &   (0.20)         &   (0.55)         &   (0.20)         &   (0.55)         &   (0.20)         \\
\addlinespace
\specialcell{Hispanic}&     2.41\sym{***}&     0.37         &     2.42\sym{***}&     0.42\sym{*}  &     2.55\sym{***}&     0.46\sym{**} &     2.57\sym{***}&     0.47\sym{**} &     2.56\sym{***}&     0.46\sym{**} \\
                &   (0.72)         &   (0.23)         &   (0.72)         &   (0.22)         &   (0.74)         &   (0.22)         &   (0.74)         &   (0.22)         &   (0.74)         &   (0.22)         \\
\addlinespace
\specialcell{Disclosure}&    31.66\sym{***}&    27.78\sym{***}&    79.07\sym{***}&    74.92\sym{***}&    13.87\sym{***}&     9.14\sym{***}&     9.16\sym{***}&     5.80\sym{***}&    31.58\sym{***}&    23.71\sym{***}\\
                &   (1.63)         &   (1.83)         &   (0.62)         &   (1.31)         &   (0.99)         &   (0.58)         &   (1.24)         &   (0.56)         &   (1.73)         &   (1.86)         \\
\addlinespace
\specialcell{Asina $ \times $ Disclosure}&    13.20\sym{***}&    16.01\sym{***}&    -3.14\sym{***}&     1.03         &     3.07         &     4.07\sym{**} &     2.24         &     3.43\sym{*}  &     8.06\sym{*}  &    11.06\sym{**} \\
                &   (2.24)         &   (2.28)         &   (0.95)         &   (1.15)         &   (1.96)         &   (1.78)         &   (2.22)         &   (1.99)         &   (4.68)         &   (4.97)         \\
\addlinespace
\specialcell{Black $ \times $ Disclosure}&    10.94\sym{***}&    12.54\sym{***}&    -1.48         &    -1.26         &     5.33\sym{***}&     7.28\sym{***}&     1.26         &     3.02         &    10.36\sym{**} &    14.74\sym{***}\\
                &   (2.32)         &   (2.25)         &   (0.94)         &   (1.26)         &   (2.00)         &   (2.04)         &   (2.32)         &   (2.39)         &   (5.03)         &   (4.92)         \\
\addlinespace
\specialcell{Hispanic $ \times $ Disclosure}&     8.65\sym{**} &    11.54\sym{***}&    -2.35\sym{**} &    -2.85         &     2.62         &     5.85\sym{***}&     0.41         &     4.45\sym{***}&    10.29\sym{***}&    10.24\sym{***}\\
                &   (4.22)         &   (3.35)         &   (1.05)         &   (2.15)         &   (2.57)         &   (1.65)         &   (2.23)         &   (1.39)         &   (3.21)         &   (3.31)         \\
\addlinespace
\specialcell{Female}&    -0.26         &    -0.22         &    -0.34         &    -0.25\sym{*}  &    -0.35         &    -0.30\sym{**} &    -0.38         &    -0.32\sym{**} &    -0.38         &    -0.32\sym{**} \\
                &   (0.23)         &   (0.14)         &   (0.23)         &   (0.14)         &   (0.23)         &   (0.14)         &   (0.23)         &   (0.14)         &   (0.23)         &   (0.14)         \\
\midrule
\specialcell{Adviser Controls}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County FE}&                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         &                  &$\pmb{\checkmark}$         \\
\specialcell{Observations}&7,022,703         &6,571,326         &7,022,703         &6,571,326         &7,022,703         &6,571,326         &7,022,703         &6,571,326         &7,022,703         &6,571,326         \\
\specialcell{\(R^2\)}&    0.006         &    0.260         &    0.011         &    0.265         &    0.001         &    0.257         &    0.001         &    0.256         &    0.001         &    0.257         \\
\specialcell{Mean of Dependent Variable}&    16.66         &    16.81         &    16.66         &    16.81         &    16.66         &    16.81         &    16.66         &    16.81         &    16.66         &    16.81         \\


==> tables/table_js_2_g_1.tex <==
                &\multicolumn{4}{c}{\specialcell{\scriptsize Job Separation (\%)}}                             \\\cmidrule(lr){2-5}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                &\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct (excl. (II))}}&\multicolumn{1}{c}{\specialcell{\scriptsize (I)}}&\multicolumn{1}{c}{\specialcell{\scriptsize (II)}}\\
\midrule
\ \specialcell{\scriptsize Female}&    -0.26\sym{**} &    -0.30\sym{**} &    -0.31\sym{**} &    -0.24\sym{*}   \\
              &   (0.13)         &   (0.13)         &   (0.13)         &   (0.13)                 \\
\addlinespace
\ \specialcell{\scriptsize Disclosure}&    29.24\sym{***}&    10.02\sym{***}&     6.44\sym{***}&    74.92\sym{***}\\
                  &   (2.20)         &   (0.73)          &   (0.62)         &   (1.40)               \\
\addlinespace
\ \specialcell{\scriptsize Female $\times$ Disclosure}&    10.94\sym{***}&    -0.03&    -1.15         &     0.87                  \\
               &   (1.57)         &   (0.90)      &   (0.83)         &   (0.80)                  \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                  \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                \\
\specialcell{\scriptsize Observations}&5,736,702         &5,736,702         &5,736,702         &5,736,702           \\
\specialcell{\scriptsize \(R^2\)}&    0.316         &    0.312        &    0.312         &    0.320                  \\
\specialcell{\scriptsize Mean of Dependent Variable}&    16.58         &    16.58         &    16.58         &    16.58           \\


==> tables/table_js_2_g_1_0.tex <==
                &\multicolumn{3}{c}{\specialcell{\scriptsize Job Separation (\%)}}                             \\\cmidrule(lr){2-4}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                &\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct (excl. event (II))}}&\multicolumn{1}{c}{\specialcell{\scriptsize event (II)}}\\
\midrule
\ \specialcell{\scriptsize Female}&    -0.26\sym{**} &    -0.30\sym{**} &      -0.24\sym{*}   \\
              &   (0.13)         &   (0.13)             &   (0.13)                 \\
\addlinespace
\ \specialcell{\scriptsize Disclosure}&    29.24\sym{***}&    10.02\sym{***}&       74.92\sym{***}\\
                  &   (2.20)         &   (0.73)                &   (1.40)               \\
\addlinespace
\ \specialcell{\scriptsize Female $\times$ Disclosure}&    10.94\sym{***}&    -0.03      &     0.87                  \\
               &   (1.57)         &   (0.90)        &   (0.80)                  \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                    \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$               &$\pmb{\checkmark}$                \\
\specialcell{\scriptsize Observations}&5,736,702         &5,736,702         &5,736,702               \\
\specialcell{\scriptsize \(R^2\)}&    0.316         &    0.312            &    0.320                  \\
\specialcell{\scriptsize Mean of Dependent Variable}&    16.58         &    16.58               &    16.58           \\


==> tables/table_js_2_g_1_1.tex <==
                &\multicolumn{3}{c}{\specialcell{Employment Separation (\%)}}                             \\\cmidrule(lr){2-4}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                &\multicolumn{1}{c}{\specialcell{Misconduct}}&\multicolumn{1}{c}{\specialcell{Misconduct (excl. Event (II))}}&\multicolumn{1}{c}{\specialcell{Event (II)}}\\
\midrule
\ \specialcell{Female}&    -0.26\sym{**} &    -0.30\sym{**} &      -0.24\sym{*}   \\
              &   (0.13)         &   (0.13)             &   (0.13)                 \\
\addlinespace
\ \specialcell{Disclosure}&    29.24\sym{***}&    10.02\sym{***}&       74.92\sym{***}\\
                  &   (2.20)         &   (0.73)                &   (1.40)               \\
\addlinespace
\ \specialcell{Female $\times$ Disclosure}&    10.94\sym{***}&    -0.03      &     0.87                  \\
               &   (1.57)         &   (0.90)        &   (0.80)                  \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                    \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$               &$\pmb{\checkmark}$                \\
\specialcell{Observations}&5,736,702         &5,736,702         &5,736,702               \\
\specialcell{\(R^2\)}&    0.316         &    0.312            &    0.320                  \\
\specialcell{Mean of Dependent Variable}&    16.58         &    16.58               &    16.58           \\


==> tables/table_js_2_g_1_2.tex <==
                &\multicolumn{3}{c}{\specialcell{Job Separation (\%)}}                             \\\cmidrule(lr){2-4}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                &\multicolumn{1}{c}{\specialcell{Misconduct}}&\multicolumn{1}{c}{\specialcell{Category B}}&\multicolumn{1}{c}{\specialcell{Category A}}\\
\midrule
\ \specialcell{Female}&    -0.26\sym{**} &    -0.30\sym{**} &      -0.24\sym{*}   \\
              &   (0.13)         &   (0.13)             &   (0.13)                 \\
\addlinespace
\ \specialcell{Disclosure}&    29.24\sym{***}&    10.02\sym{***}&       74.92\sym{***}\\
                  &   (2.20)         &   (0.73)                &   (1.40)               \\
\addlinespace
\ \specialcell{Female $\times$ Disclosure}&    10.94\sym{***}&    -0.03      &     0.87                  \\
               &   (1.57)         &   (0.90)        &   (0.80)                  \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                    \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$               &$\pmb{\checkmark}$                \\
\specialcell{Observations}&5,736,702         &5,736,702         &5,736,702               \\
\specialcell{\(R^2\)}&    0.316         &    0.312            &    0.320                  \\
\specialcell{Mean of Dependent Variable}&    16.58         &    16.58               &    16.58           \\


==> tables/table_js_2_g_2.tex <==
                &\multicolumn{3}{c}{\specialcell{\scriptsize Job Separation (\%)}}                             \\\cmidrule(lr){2-4}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                &\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct (excl. event (II))}}&\multicolumn{1}{c}{\specialcell{\scriptsize event (II)}}\\
\midrule
\ \specialcell{\scriptsize Female}&    -0.26\sym{**} &    -0.30\sym{**} &      -0.24\sym{*}   \\
              &   (0.13)         &   (0.13)             &   (0.13)                 \\
\addlinespace
\ \specialcell{\scriptsize Disclosure}&    29.24\sym{***}&    10.02\sym{***}&       74.92\sym{***}\\
                  &   (2.20)         &   (0.73)                &   (1.40)               \\
\addlinespace
\ \specialcell{\scriptsize Female $\times$ Disclosure}&    10.94\sym{***}&    -0.03      &     0.87                  \\
               &   (1.57)         &   (0.90)        &   (0.80)                  \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                    \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$               &$\pmb{\checkmark}$                \\
\specialcell{\scriptsize Observations}&5,736,702         &5,736,702         &5,736,702               \\
\specialcell{\scriptsize \(R^2\)}&    0.316         &    0.312            &    0.320                  \\
\specialcell{\scriptsize Mean of Dependent Variable}&    16.58         &    16.58               &    16.58           \\


==> tables/table_js_2_r_1_0.tex <==
                &\multicolumn{4}{c}{\specialcell{\scriptsize Job Separation (\%)}}                             \\\cmidrule(lr){2-5}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                &\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct (excl. (II))}}&\multicolumn{1}{c}{\specialcell{\scriptsize (I)}}&\multicolumn{1}{c}{\specialcell{\scriptsize (II)}}\\
\midrule
\specialcell{Minority}&     0.57\sym{***}&       0.66\sym{***}&     0.67\sym{***}&     0.63\sym{***} \\
                &   (0.19)               &   (0.18)         &   (0.18)         &   (0.18)         \\
\addlinespace
\specialcell{Disclosure}&    29.14\sym{***}&     9.36\sym{***}&     5.89\sym{***}&    75.36\sym{***}\\
                &   (2.09)            &   (0.69)         &   (0.64)       &   (1.39)             \\
\addlinespace
\specialcell{Minority $ \times $ Disclosure}&    13.76\sym{***}         &     6.41\sym{***}&     4.41\sym{***}&    -1.52\\
                &   (2.48)             &   (1.40)         &   (1.30)     &   (1.29)             \\
\addlinespace
\specialcell{Female}&    -0.23\sym{*}   &    -0.31\sym{**} &    -0.33\sym{**}  &    -0.25\sym{*} \\
                &   (0.13)              &   (0.13)         &   (0.13)         &   (0.13)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$             \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$            &$\pmb{\checkmark}$         \\
\specialcell{Observations}&5,736,702         &5,736,702         &5,736,702         &5,736,702        \\
\specialcell{\(R^2\)}&    0.316             &    0.312         &    0.312        &    0.320           \\
\specialcell{Mean of Dependent Variable}&    16.58         &    16.58         &    16.58         &    16.58               \\


==> tables/table_js_2_r_1_1.tex <==
                &\multicolumn{3}{c}{\specialcell{Employment Separation (\%)}}                             \\\cmidrule(lr){2-4}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                &\multicolumn{1}{c}{\specialcell{Misconduct}}&\multicolumn{1}{c}{\specialcell{Misconduct (excl. Event (II))}}&\multicolumn{1}{c}{\specialcell{Event (II)}}\\
\midrule
\specialcell{Minority}&     0.57\sym{***}&       0.66\sym{***}&     0.63\sym{***} \\
                &   (0.19)               &   (0.18)              &   (0.18)         \\
\addlinespace
\specialcell{Disclosure}&    29.14\sym{***}&     9.36\sym{***}&       75.36\sym{***}\\
                &   (2.09)            &   (0.69)            &   (1.39)             \\
\addlinespace
\specialcell{Disclosure $ \times $ Minority}&    13.76\sym{***}         &     6.41\sym{***}&       -1.52\\
                &   (2.48)             &   (1.40)           &   (1.29)             \\
\addlinespace
\specialcell{Female}&    -0.23\sym{*}   &    -0.31\sym{**}   &    -0.25\sym{*} \\
                &   (0.13)              &   (0.13)           &   (0.13)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                  \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                \\
\specialcell{Observations}&5,736,702         &5,736,702            &5,736,702        \\
\specialcell{\(R^2\)}&    0.316             &    0.312            &    0.320           \\
\specialcell{Mean of Dependent Variable}&    16.58              &    16.58         &    16.58               \\


==> tables/table_js_2_r_1_2.tex <==
                &\multicolumn{3}{c}{\specialcell{Job Separation (\%)}}                             \\\cmidrule(lr){2-4}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                &\multicolumn{1}{c}{\specialcell{Misconduct}}&\multicolumn{1}{c}{\specialcell{Category B}}&\multicolumn{1}{c}{\specialcell{Category A}}\\
\midrule
\specialcell{Minority}&     0.57\sym{***}&       0.66\sym{***}&     0.63\sym{***} \\
                &   (0.19)               &   (0.18)              &   (0.18)         \\
\addlinespace
\specialcell{Disclosure}&    29.14\sym{***}&     9.36\sym{***}&       75.36\sym{***}\\
                &   (2.09)            &   (0.69)            &   (1.39)             \\
\addlinespace
\specialcell{Disclosure $ \times $ Minority}&    13.76\sym{***}         &     6.41\sym{***}&       -1.52\\
                &   (2.48)             &   (1.40)           &   (1.29)             \\
\addlinespace
\specialcell{Female}&    -0.23\sym{*}   &    -0.31\sym{**}   &    -0.25\sym{*} \\
                &   (0.13)              &   (0.13)           &   (0.13)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                  \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$                \\
\specialcell{Observations}&5,736,702         &5,736,702            &5,736,702        \\
\specialcell{\(R^2\)}&    0.316             &    0.312            &    0.320           \\
\specialcell{Mean of Dependent Variable}&    16.58              &    16.58         &    16.58               \\


==> tables/table_js_2_r_2.tex <==
                &\multicolumn{4}{c}{\specialcell{\scriptsize Job Separation (\%)}}                             \\\cmidrule(lr){2-5}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                &\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct}}&\multicolumn{1}{c}{\specialcell{\scriptsize Misconduct (excl. (II))}}&\multicolumn{1}{c}{\specialcell{\scriptsize (I)}}&\multicolumn{1}{c}{\specialcell{\scriptsize (II)}}\\
\midrule
\specialcell{\scriptsize Disclosure}&    41.19\sym{***}&     4.62\sym{***}&     5.59\sym{***}&    77.39\sym{***}&    29.19\sym{***}\\
                &   (3.85)         &   (1.24)         &   (1.50)         &   (1.63)         &   (6.65)         \\
\addlinespace
\specialcell{\scriptsize Hispanic}&    -0.51\sym{***}&    -0.48\sym{***}&    -0.47\sym{***}&    -0.48\sym{***}&    -0.48\sym{***}\\
                &   (0.18)         &   (0.17)         &   (0.17)         &   (0.17)         &   (0.17)         \\
\addlinespace
\specialcell{\scriptsize Asian}&     0.75\sym{***}&     0.83\sym{***}&     0.84\sym{***}&     0.77\sym{***}&     0.83\sym{***}\\
                &   (0.25)         &   (0.25)         &   (0.25)         &   (0.25)         &   (0.25)         \\
\addlinespace
\specialcell{\scriptsize Black}&     0.08         &     0.10         &     0.10         &     0.10         &     0.11         \\
                &   (0.23)         &   (0.23)         &   (0.23)         &   (0.23)         &   (0.23)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Hispanic}&     8.25\sym{**} &     4.64         &     1.66         &    -6.82\sym{**} &    20.24\sym{***}\\
                &   (3.33)         &   (3.24)         &   (4.64)         &   (2.96)         &   (6.65)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Asian}&     9.52\sym{***}&     1.34         &     0.27         &    -5.17\sym{**} &    26.92\sym{*}  \\
                &   (3.23)         &   (4.24)         &   (3.93)         &   (2.38)         &  (14.48)         \\
\addlinespace
\specialcell{\scriptsize Disclosure $ \times $ Black}&     1.99         &     0.78         &     4.33         &    -2.84         &    -9.84         \\
                &   (6.80)         &   (8.33)         &  (13.88)         &   (7.80)         &  (14.87)         \\
\midrule
\specialcell{\scriptsize Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{\scriptsize Observations}&1,417,189         &1,417,189         &1,417,189         &1,417,189         &1,417,189         \\
\specialcell{\scriptsize \(R^2\)}&    0.337         &    0.333         &    0.333         &    0.339         &    0.334         \\
\specialcell{\scriptsize Mean of Dependent Variable}&    16.07         &    16.07         &    16.07         &    16.07         &    16.07         \\



==> tables/table_js_3_r_0.tex <==
                &\multicolumn{5}{c}{\specialcell{Job Separation (\%)}}                                         \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                &\multicolumn{1}{c}{\specialcell{Misconduct}}&\multicolumn{1}{c}{\specialcell{Misconduct (excl. Emp.Sep.)}}&\multicolumn{1}{c}{\specialcell{Cus.Set.}}&\multicolumn{1}{c}{\specialcell{Emp.Sep.}}&\multicolumn{1}{c}{\specialcell{Reg.}}\\
\midrule
\specialcell{Disclosure}&    29.44\sym{***}&     4.41\sym{***}&     5.98\sym{***}&    75.53\sym{***}&    25.35\sym{***}\\
                &   (2.14)         &   (0.46)         &   (0.64)         &   (1.38)         &   (2.31)         \\
\addlinespace
\specialcell{Hispanic}&    -0.03         &     0.06         &     0.06         &     0.04         &     0.06         \\
                &   (0.18)         &   (0.17)         &   (0.17)         &   (0.17)         &   (0.17)         \\
\addlinespace
\specialcell{Asian}&     0.73\sym{***}&     0.84\sym{***}&     0.83\sym{***}&     0.78\sym{***}&     0.84\sym{***}\\
                &   (0.20)         &   (0.19)         &   (0.19)         &   (0.20)         &   (0.19)         \\
\addlinespace
\specialcell{Black}&     0.26\sym{*}  &     0.32\sym{**} &     0.31\sym{**} &     0.28\sym{*}  &     0.31\sym{**} \\
                &   (0.15)         &   (0.15)         &   (0.15)         &   (0.15)         &   (0.15)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Hispanic}&    10.18\sym{***}&     2.79\sym{**} &     2.85\sym{**} &    -3.72\sym{*}  &    11.18\sym{***}\\
                &   (3.04)         &   (1.12)         &   (1.15)         &   (1.94)         &   (2.97)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Asian}&    14.65\sym{***}&     1.04         &     4.32\sym{**} &    -0.03         &    13.92\sym{***}\\
                &   (2.18)         &   (1.64)         &   (1.82)         &   (1.08)         &   (4.66)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Black}&     5.76\sym{**} &     0.67         &     1.40         &    -2.11         &     4.37         \\
                &   (2.42)         &   (2.58)         &   (2.99)         &   (2.15)         &   (6.12)         \\
\addlinespace
\specialcell{Female}&    -0.23\sym{*}  &    -0.33\sym{**} &    -0.33\sym{**} &    -0.26\sym{**} &    -0.33\sym{**} \\
                &   (0.13)         &   (0.13)         &   (0.13)         &   (0.13)         &   (0.13)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Observations}&5,736,702         &5,736,702         &5,736,702         &5,736,702         &5,736,702         \\
\specialcell{\(R^2\)}&    0.316         &    0.312         &    0.312         &    0.320         &    0.312         \\
\specialcell{Mean of Dependent Variable}&    16.58         &    16.58         &    16.58         &    16.58         &    16.58         \\


==> tables/table_js_3_r_1.tex <==
                &\multicolumn{3}{c}{\specialcell{Employment Separation (\%)}}                             \\\cmidrule(lr){2-4}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                &\multicolumn{1}{c}{\specialcell{Misconduct}}&\multicolumn{1}{c}{\specialcell{Misconduct (excl. Event (II))}}&\multicolumn{1}{c}{\specialcell{Event (II)}}\\
\midrule
\specialcell{Disclosure}&    29.44\sym{***}&     4.41\sym{***}&     75.53\sym{***}\\
                &   (2.14)         &   (0.46)            &   (1.38)                \\
\addlinespace
\specialcell{Hispanic}&    -0.03         &     0.06         &         0.04             \\
                &   (0.18)         &   (0.17)              &   (0.17)            \\
\addlinespace
\specialcell{Asian}&     0.73\sym{***}&     0.84\sym{***}&     0.78\sym{***}\\
                &   (0.20)         &   (0.19)          &   (0.20)               \\
\addlinespace
\specialcell{Black}&     0.26\sym{*}  &     0.32\sym{**}  &     0.28\sym{*} \\
                &   (0.15)         &   (0.15)                &   (0.15)          \\
\addlinespace
\specialcell{Disclosure $ \times $ Hispanic}&    10.18\sym{***}&     2.79\sym{**}  &    -3.72\sym{*}  \\
                &   (3.04)         &   (1.12)                &   (1.94)              \\
\addlinespace
\specialcell{Disclosure $ \times $ Asian}&    14.65\sym{***}&     1.04        &    -0.03        \\
                &   (2.18)         &   (1.64)               &   (1.08)             \\
\addlinespace
\specialcell{Disclosure $ \times $ Black}&     5.76\sym{**}       &     1.40         &    -2.11               \\
                &   (2.42)         &   (2.58)               &   (2.15)       \\
\addlinespace
\specialcell{Female}&    -0.23\sym{*}  &    -0.33\sym{**} &    -0.26\sym{**}  \\
                &   (0.13)         &   (0.13)            &   (0.13)              \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$               \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$               &$\pmb{\checkmark}$         \\
\specialcell{Observations}&5,736,702         &5,736,702         &5,736,702               \\
\specialcell{\(R^2\)}&    0.316         &    0.312               &    0.320                \\
\specialcell{Mean of Dependent Variable}&    16.58         &    16.58         &    16.58               \\


==> tables/table_js_r_1.tex <==
                &\multicolumn{5}{c}{\specialcell{Job Separation (\%)}}                                         \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                &\multicolumn{1}{c}{\specialcell{Misconduct}}&\multicolumn{1}{c}{\specialcell{Misconduct (excl. Emp.Sep.)}}&\multicolumn{1}{c}{\specialcell{Cus.Set.}}&\multicolumn{1}{c}{\specialcell{Emp.Sep.}}&\multicolumn{1}{c}{\specialcell{Reg.}}\\
\midrule
\specialcell{Disclosure}&    29.44\sym{***}&     4.41\sym{***}&     5.98\sym{***}&    75.53\sym{***}&    25.35\sym{***}\\
                &   (2.14)         &   (0.46)         &   (0.64)         &   (1.38)         &   (2.31)         \\
\addlinespace
\specialcell{Hispanic}&    -0.03         &     0.06         &     0.06         &     0.04         &     0.06         \\
                &   (0.18)         &   (0.17)         &   (0.17)         &   (0.17)         &   (0.17)         \\
\addlinespace
\specialcell{Asian}&     0.73\sym{***}&     0.84\sym{***}&     0.83\sym{***}&     0.78\sym{***}&     0.84\sym{***}\\
                &   (0.20)         &   (0.19)         &   (0.19)         &   (0.20)         &   (0.19)         \\
\addlinespace
\specialcell{Black}&     0.26\sym{*}  &     0.32\sym{**} &     0.31\sym{**} &     0.28\sym{*}  &     0.31\sym{**} \\
                &   (0.15)         &   (0.15)         &   (0.15)         &   (0.15)         &   (0.15)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Hispanic}&    10.18\sym{***}&     2.79\sym{**} &     2.85\sym{**} &    -3.72\sym{*}  &    11.18\sym{***}\\
                &   (3.04)         &   (1.12)         &   (1.15)         &   (1.94)         &   (2.97)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Asian}&    14.65\sym{***}&     1.04         &     4.32\sym{**} &    -0.03         &    13.92\sym{***}\\
                &   (2.18)         &   (1.64)         &   (1.82)         &   (1.08)         &   (4.66)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Black}&     5.76\sym{**} &     0.67         &     1.40         &    -2.11         &     4.37         \\
                &   (2.42)         &   (2.58)         &   (2.99)         &   (2.15)         &   (6.12)         \\
\addlinespace
\specialcell{Female}&    -0.23\sym{*}  &    -0.33\sym{**} &    -0.33\sym{**} &    -0.26\sym{**} &    -0.33\sym{**} \\
                &   (0.13)         &   (0.13)         &   (0.13)         &   (0.13)         &   (0.13)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Observations}&5,736,702         &5,736,702         &5,736,702         &5,736,702         &5,736,702         \\
\specialcell{\(R^2\)}&    0.316         &    0.312         &    0.312         &    0.320         &    0.312         \\
\specialcell{Mean of Dependent Variable}&    16.58         &    16.58         &    16.58         &    16.58         &    16.58         \\


==> tables/table_js_r_2.tex <==
                &\multicolumn{5}{c}{\specialcell{Job Separation (\%)}}                                         \\\cmidrule(lr){2-6}
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                &\multicolumn{1}{c}{\specialcell{Misconduct}}&\multicolumn{1}{c}{\specialcell{Misconduct (excl. Emp.Sep.)}}&\multicolumn{1}{c}{\specialcell{Cus.Set.}}&\multicolumn{1}{c}{\specialcell{Emp.Sep.}}&\multicolumn{1}{c}{\specialcell{Reg.}}\\
\midrule
\specialcell{Disclosure}&    29.14\sym{***}&     4.28\sym{***}&     5.88\sym{***}&    75.35\sym{***}&    25.21\sym{***}\\
                &   (2.09)         &   (0.44)         &   (0.64)         &   (1.39)         &   (2.28)         \\
\addlinespace
\specialcell{Hispanic}&     0.18         &     0.27         &     0.27         &     0.24         &     0.27         \\
                &   (0.22)         &   (0.21)         &   (0.21)         &   (0.21)         &   (0.21)         \\
\addlinespace
\specialcell{Asian}&     0.79\sym{***}&     0.91\sym{***}&     0.90\sym{***}&     0.84\sym{***}&     0.90\sym{***}\\
                &   (0.24)         &   (0.23)         &   (0.23)         &   (0.23)         &   (0.23)         \\
\addlinespace
\specialcell{Black}&     0.98\sym{***}&     1.07\sym{***}&     1.07\sym{***}&     1.04\sym{***}&     1.07\sym{***}\\
                &   (0.21)         &   (0.21)         &   (0.21)         &   (0.21)         &   (0.21)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Hispanic}&    12.17\sym{***}&     3.80\sym{***}&     4.52\sym{***}&    -2.83         &    11.12\sym{***}\\
                &   (3.43)         &   (1.42)         &   (1.52)         &   (2.04)         &   (3.48)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Asian}&    17.32\sym{***}&     1.88         &     4.52\sym{**} &     0.97         &    13.98\sym{**} \\
                &   (2.35)         &   (2.02)         &   (2.27)         &   (1.25)         &   (5.83)         \\
\addlinespace
\specialcell{Disclosure $ \times $ Black}&    13.37\sym{***}&     5.51\sym{***}&     4.12         &    -1.61         &    14.67\sym{**} \\
                &   (2.13)         &   (1.98)         &   (2.61)         &   (1.47)         &   (5.75)         \\
\addlinespace
\specialcell{Female}&    -0.24\sym{*}  &    -0.34\sym{**} &    -0.33\sym{**} &    -0.26\sym{**} &    -0.33\sym{**} \\
                &   (0.13)         &   (0.13)         &   (0.13)         &   (0.13)         &   (0.13)         \\
\midrule
\specialcell{Adviser Controls}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Firm $\times$ Year $\times$ County $\times$ License FE}&$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         &$\pmb{\checkmark}$         \\
\specialcell{Observations}&5,736,702         &5,736,702         &5,736,702         &5,736,702         &5,736,702         \\
\specialcell{\(R^2\)}&    0.316         &    0.312         &    0.312         &    0.320         &    0.312         \\
\specialcell{Mean of Dependent Variable}&    16.58         &    16.58         &    16.58         &    16.58         &    16.58         \\


==> tables/table_ss_1.tex <==
\multicolumn{7}{c}{\specialcell{\bf A. Adviser Characteristics}}\\
\midrule
&\multicolumn{3}{c}{\specialcell{Male}}&\multicolumn{3}{c}{\specialcell{Female}}\\\cmidrule(lr){2-4}\cmidrule(lr){5-7}
          &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
          &\multicolumn{1}{c}{\specialcell{All}}&\multicolumn{1}{c}{\specialcell{Majority}}&\multicolumn{1}{c}{\specialcell{Minority}}&\multicolumn{1}{c}{\specialcell{All}}&\multicolumn{1}{c}{\specialcell{Majority}}&\multicolumn{1}{c}{\specialcell{Minority}}\\
\midrule
{\specialcell{\bf Employment History and Status:}}&         &         &         &         &         &         \\
\ \specialcell{Experience (years)}&     13.4&     13.9&      9.3&     10.8&     11.2&      8.1\\
\ \specialcell{Tenure (years)}&      6.3&      6.5&      4.6&      5.7&      5.9&      4.5\\
\hline {\specialcell{\bf Licenses/Industry Exams}}&         &         &         &         &         &         \\
\ \specialcell{Series 63 (General Securities Agent)}&     74.3&     74.8&     70.4&     68.7&     68.9&     67.9\\
\ \specialcell{Series 7 (General Securities Representative)}&     69.0&     69.8&     61.4&     62.4&     63.6&     55.1\\
\ \specialcell{Series 6 (Insurance and Annuities)}&     35.5&     35.2&     38.6&     42.4&     42.0&     45.2\\
\ \specialcell{Series 65/66 (Investment Adviser)}&     42.1&     43.4&     31.0&     34.8&     36.0&     27.1\\
\ \specialcell{Series 24 (Principal/Supervisory Management)}&     15.4&     16.0&     10.3&     10.6&     11.2&      7.1\\
\hline \ \specialcell{Total Number of Licenses}&      2.9&      2.9&      2.5&      2.5&      2.6&      2.3\\
\midrule
\multicolumn{7}{c}{\specialcell{\bf B. Disclosure Event Incidence}}\\
\midrule
{\specialcell{\bf Misconduct Related Disclosure Events} (\%):}&         &         &         &         &         &         \\
\ \specialcell{Customer Disputes - Settled}&     0.37&     0.37&     0.34&     0.13&     0.13&     0.12\\
\ \specialcell{Employment Separation After Allegations}&     0.23&     0.21&     0.37&     0.15&     0.14&     0.24\\
\ \specialcell{Regulatory - Final}&     0.12&     0.12&     0.12&     0.04&     0.04&     0.04\\
\ \specialcell{Criminal Disposition - Final}&     0.03&     0.03&     0.04&     0.01&     0.01&     0.01\\
\ \specialcell{Customer Disputes - Award/Judgment}&     0.02&     0.02&     0.02&     0.01&     0.01&     0.00\\
\ \specialcell{Civil - Final}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Any Misconduct Related Disclosure}&     0.71&     0.70&     0.82&     0.32&     0.31&     0.39\\
\hline {\specialcell{\bf Other Disclosure Events} (\%):}&         &         &         &         &         &         \\
\ \specialcell{Financial - Final}&     0.42&     0.40&     0.51&     0.49&     0.47&     0.58\\
\ \specialcell{Judgment/Lien}&     0.33&     0.33&     0.39&     0.20&     0.18&     0.28\\
\ \specialcell{Customer Disputes - Denied}&     0.33&     0.34&     0.27&     0.14&     0.14&     0.14\\
\ \specialcell{Customer Disputes - Closed-No Action}&     0.07&     0.07&     0.07&     0.02&     0.02&     0.03\\
\ \specialcell{Financial - Pending}&     0.04&     0.04&     0.05&     0.06&     0.05&     0.07\\
\ \specialcell{Customer Disputes - Pending}&     0.06&     0.06&     0.11&     0.02&     0.02&     0.03\\
\ \specialcell{Customer Disputes - Withdrawn}&     0.02&     0.02&     0.02&     0.01&     0.01&     0.01\\
\ \specialcell{Criminal - Pending}&     0.01&     0.01&     0.01&     0.00&     0.00&     0.01\\
\ \specialcell{Investigation}&     0.01&     0.01&     0.01&     0.00&     0.00&     0.00\\
\ \specialcell{Regulatory - Pending}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Civil - Pending}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Customer Disputes - Final}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Customer Disputes - Dismissed}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Civil Bond}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Regulatory - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Criminal - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\ \specialcell{Civil - On Appeal}&     0.00&     0.00&     0.00&     0.00&     0.00&     0.00\\
\hline  \specialcell{\bf Total} (\%):&     1.89&     1.86&     2.13&     1.21&     1.17&     1.46\\
\midrule
Observations&5,753,021&5,150,027&  542,597&2,153,206&1,843,251&  267,990\\

